Distributionally Robust Martingale Optimal Transport

We study the problem of bounding path-dependent expectations (within any finite time horizon $d$) over the class of discrete-time martingales whose marginal distributions lie within a prescribed tolerance of a given collection of benchmark marginal distributions. This problem is a relaxation of the martingale optimal transport (MOT) problem and is motivated by applications to super-hedging in financial markets. We show that the empirical version of our relaxed MOT problem can be approximated within $O\left( n^{-1/2}\right)$ error where $n$ is the number of samples of each of the individual marginal distributions (generated independently) and using a suitably constructed finite-dimensional linear programming problem.

==> approximation_compact.tex <==
In section \ref{subsec.stability} we proved that \eqref{eq.empiricalworstcase} is indeed concentrate to \eqref{eq.worstcase} with rate $\calO(1/\sqrt{n})$. 
However,  \eqref{eq.empiricalworstcase} is still computationally intractable as an infinite dimensional LP. A natural way to over come this difficulty is to approximate \eqref{eq.empiricalworstcase} via a proper discretization. In this section we propose such an approximation scheme to approximately compute \eqref{eq.empiricalworstcase} within arbitrary prefixed error. 

For technical reasons, we assume in this section that each $\Omega_i$ (the support of $\mu_i$) is a closed interval $[a_i, b_i]$ in $\RR$ with length $l_i=b_i - a_i$, we have $a_1\geq\cdots\geq a_d$ and $b_1\leq\cdots\leq b_d$ as a direct consequence of Assumption \ref{aspn.compact_support}.  For each $i\in\left\lbrace 1,\cdots,d \right\rbrace$, denoted by $\Omega_{i}^{(N)}$, the $N$-fold discretization of $\Omega_i = [a_i, b_i]$ is defined by

\begin{equation}
\Omega_{i}^{(N)} = \left\lbrace a_i + \frac{k(b_i-a_i)}{N}: k=0, 1,\cdots,N\right\rbrace
\end{equation}

The first step is to show that any martingale probability measure $\pi$ on $\Omega = \Omega_1\times\cdots\times\Omega_d$  can be approximated by some ``almost martingale probability measure" $\pi^{(N)}$ with finite support. almost-martingale measure, which is a relaxation of martingale measure. 

\begin{definition}
($\delta$-martingale probability measure) A probability measure $\pi$ on $\RR^d$ is a $\delta$-martingale probability measure if
\[
\left|\EE_{\bX\sim\pi}\left[X_{k+1}|\calF_k\right] - X_k\right| \leq \delta \qquad \pi - a.s.
\]
for all $k=1,2,\cdots,d-1$, where $\calF_k=\sigma(X_1,\cdots,X_k)$ is the canonical filtration. Moreover, we define $M_{(\mu_1,\cdots,\mu_d)}(\delta)$ to be the set of $\delta$-martingale probability measures that contained in $\Pi(\mu_1,\cdots,\mu_d)$. 
\end{definition}
Now we are ready to state and prove the following lemma, which construct  discrete ``almost" martingales that arbitrarily close to a given martingale.
\begin{lemma}\label{lemma.discretize}
With Assumption \ref{aspn.compact_support}, given $\varepsilon>0$, for any martingale probability measure $\pi$ on $\Omega=\Omega_1\times\cdots\times\Omega_d$ and integer $N$, there exist a $\widetilde{L}/N$-martingale probability measure $\pi^{(N)}$ such that 
\begin{enumerate}
\item [\emph{(1)}] $\pi^{(N)}_i$ supported on $\Omega_i^{(N)}$ for all $i\in\left\lbrace 1,2,\cdots, d\right\rbrace$
\item [\emph{(2)}] $\calW\left(\pi,\pi^{(N)}\right)\leq\frac{\widetilde{L}\sqrt{d}}{N}$, i.e., $\pi$ and $\pi^{(N)}$ are close in Wasserstein distance, where $\widetilde{L}:=\max_{1\leq i\leq d}l_i$.
\end{enumerate}
\end{lemma}

\begin{proof}
Let us  introduce some useful notations. For any $1\leq i\leq d$, $k_i\in \ZZ$, we define 
\begin{equation}
I_{i,k_i}^{(-1)} := \left[a_i + \frac{(k_i - 1)l_i}{N}, a_i + \frac{k_il_i}{N}\right], \qquad I_{i,k_i}^{(+1)} := \left[a_i + \frac{k_il_i}{N}, a_i + \frac{(k_i + 1)l_i}{N}\right]
\end{equation}
and 
\begin{equation}
g_{i,k_i}^{(-1)}(x_i):= \frac{1}{l_i}\left(Nx_i - Na_i - (k_i - 1)l_i\right), \qquad g_{i,k_i}^{(+1)}(x_i) := \frac{1}{l_i}\left(Na_i + (k_i + 1)l_i - Nx_i\right)
\end{equation}
Note that $g_{i,k_i}^{(-1)}(x_i)$ and $g_{i,k_i}^{(+1)}(x_i)$ are non-negative, and we also have $g_{i,k_i}^{(-1)}(x_i) + g_{i,k_i-1}^{(+1)}(x_i) =1$. Let $\pi$ be a martingale probability measure on $\Omega$, we define a probability measure $\pi^{(N)}$ supported on $\Omega$ as follows: 
\begin{equation}\label{eq.discrete_pi}
\pi^{(N)}\left(a_1+\frac{k_1l_1}{N},\cdots, a_d+\frac{k_dl_d}{N}\right) := \sum_{(t_1,\cdots, t_d)\in\left\lbrace -1, +1\right\rbrace^d}\int_{\prod\limits_{i=1}^dI_{i,k_i}^{(t_i)}}\prod\limits_{i=1}^dg_{i,k_i}^{(t_i)}(x_i)\pi(dx_1,\cdots, dx_d)
\end{equation}
for all $0\leq k_i\leq N$, $1\leq i\leq d$. We first verify that $\pi^{(N)}$ is indeed a probability measure. Fix $k_2,\cdots, k_d$ and sum over $k_1$ yields (note that $\pi \equiv 0$ on $\Omega^c$)
\begin{align*}
&\sum_{0\leq k_1 \leq N} \pi^{(N)}\left(a_1+\frac{k_1l_1}{N},\cdots, a_d+\frac{k_dl_d}{N}\right) \\
= & \sum_{(t_2,\cdots, t_d)\in\left\lbrace -1, +1\right\rbrace^{d-1}}\int_{\prod\limits_{i=2}^dI_{i,k_i}^{(t_i)}}\prod\limits_{i=2}^dg_{i,k_i}^{(t_i)}\left[\sum_{ k_1}\left(\int_{I_{1,k_1}^{(-1)}}g_{1,k_1}^{(-1)}(x_1)+ \int_{I_{1,k_1}^{(+1)}}g_{1,k_1}^{(+1)}(x_1)\right)\pi(dx_1,\cdots, dx_d)\right]\\
=& \sum_{(t_2,\cdots, t_d)\in\left\lbrace -1, +1\right\rbrace^{d-1}}\int_{\prod\limits_{i=2}^dI_{i,k_i}^{(t_i)}}\prod\limits_{i=2}^dg_{i,k_i}^{(t_i)}\left[\sum_{k_1}\int_{I_{1,k_1}^{(-1)}}\left(g_{1,k_1}^{(-1)}(x_1) + g_{1,k_1-1}^{(+1)}(x_i)\right)\pi(dx_1,\cdots, dx_d)\right]\\
=& \sum_{(t_2,\cdots, t_d)\in\left\lbrace -1, +1\right\rbrace^{d-1}}\int_{\prod\limits_{i=2}^dI_{i,k_i}^{(t_i)}}\prod\limits_{i=2}^dg_{i,k_i}^{(t_i)}\left[\sum_{k_1}\int_{I_{1,k_1}^{(-1)}}\pi(dx_1,\cdots, dx_d)\right]\\
=& \sum_{(t_2,\cdots, t_d)\in\left\lbrace -1, +1\right\rbrace^{d-1}}\int_{\prod\limits_{i=2}^dI_{i,k_i}^{(t_i)}}\prod\limits_{i=2}^dg_{i,k_i}^{(t_i)}(x_i)\pi_{2:d}(dx_2,\cdots,dx_d)
\end{align*}
where $\pi_{2:d}(dx_2,\cdots, dx_d) = \int_{\Omega_1}\pi(dx_1,\cdots,dx_d)$ is also a probability measure. 
Therefore we can sum over $k_i$ $(1\leq i\leq d)$
iteratively and get 
\begin{equation}
\sum_{1\leq i\leq d, 0\leq k_i \leq N} \pi^{(N)}\left(a_1+\frac{k_1l_1}{N},\cdots, a_d+\frac{k_dl_d}{N}\right) = 1
\end{equation}
Furthermore, from the above arguments we have the $i$th $(1\leq i\leq d)$ marginal of $\pi^{(N)}$ is 
\begin{equation}
\pi_i^{(N)}\left(a_i + \frac{k_il_i}{N}\right) = \int_{I_{i,k_i}^{(-1)}}g_{i,k_i}^{(-1)}(x_i)\pi_i(dx_i) + \int_{I_{i,k_i}^{(+1)}}g_{i,k_i}^{(+1)}(x_i)\pi_i(dx_i), \qquad 0\leq k_i\leq N
\end{equation}
where $\pi_i$ is the $i$th marginal of $\pi$. Next we show that $\pi$ and $\pi^{(N)}$ are close in Wasserstein distance. Note that for any 1$-$Lipschitz function $\phi$, we have
{\small{
\begin{align*}
&\int \phi d\pi^{(N)} - \int\phi d\pi \\
= &\sum_{1\leq i\leq d, 0\leq k_i \leq N} \phi\left(a_1+\frac{k_1l_1}{N}, \cdots, a_d+\frac{k_dl_d}{N}\right)\pi^{(N)}\left(a_1+\frac{k_1l_1}{N},\cdots, a_d+\frac{k_dl_d}{N}\right) - \int\phi d\pi\\
= & \sum_{k_1,\cdots, k_d}\int_{\prod\limits_{i=1}^dI_{i,k_i}^{(-1)}}\sum_{(s_1,\cdots,s_d)\in\{0,1\}^d}\prod\limits_{i=1}^dg_{i,k_i-s_i}^{(2s_i-1)}(x_i)\left[\phi\left(\left\lbrace a_i+\frac{(k_i-s_i)l_i}{N}\right\rbrace_{i=1}^d\right) -\phi\left(\left\lbrace x_i\right\rbrace_{i=1}^d\right)\right]\pi(dx_1,\cdots,dx_d)
\end{align*}
}}
where  $\sum_{(s_1,\cdots,s_d)\in\{0,1\}^d}\prod\limits_{i=1}^dg_{i,k_i-s_i}^{(2s_i-1)}(x_i) = \prod_{i=1}^d\left(g_{i,k_i}^{(-1)}(x_i) + g_{i,k_i-1}^{(+1)}(x_i)\right) = 1$ is used in the last step. 

\noindent For any $(x_1,\cdots, x_d)\in \prod\limits_{i=1}^dI_{i,k_i}^{(-1)}$ and $(s_1,\cdots,s_d)\in\{0,1\}^d$, by Lipschitz property of $\phi$ we get
\begin{equation}
\left|\phi\left(\left\lbrace a_i+\frac{(k_i-s_i)l_i}{N}\right\rbrace_{i=1}^d\right) -\phi\left(\left\lbrace x_i\right\rbrace_{i=1}^d\right)\right|\leq \frac{\widetilde{L}\sqrt{d}}{N}
\end{equation}
Consequently
\begin{align*}
\calW\left(\pi^{(N)},\pi\right) &= \inf_{\phi\in\textrm{Lip}_1}\left\lbrace \int \phi d\pi^{(N)} - \int\phi d\pi \right\rbrace\\
&\leq \frac{\widetilde{L}\sqrt{d}}{N}\sum_{k_1,\cdots, k_d}\int_{\prod\limits_{i=1}^dI_{i,k_i}^{(-1)}}\sum_{(s_1,\cdots,s_d)\in\{0,1\}^d}\prod\limits_{i=1}^dg_{i,k_i-s_i}^{(2s_i-1)}(x_i)\pi(dx_1,\cdots,dx_d)\\
&\leq \frac{\widetilde{L}\sqrt{d}}{N}
\end{align*}
Finally, we check that $\pi^{(N)}$ is a $\widetilde{L}/N-$ martingale measure, that is, for all $1\leq j\leq d-1$, 
{\small
\begin{equation}\label{eq.delta_martingale}
\left|\sum_{0\leq k_{j+1}\leq N}\left[\left(a_{j+1} + \frac{k_{j+1}l_{j+1}}{N}\right) - \left(a_j + \frac{k_jl_j}{N}\right)\right]\frac{\pi^{(N)}_{1:j+1}\left(a_1+\frac{k_1l_1}{N},\cdots, a_{j+1}+\frac{k_{j+1}l_{j+1}}{N}\right)}{\pi^{(N)}_{1:j}\left(a_1+\frac{k_1l_1}{N},\cdots, a_{j}+\frac{k_{j}l_{j}}{N}\right)}\right|\leq \frac{\widetilde{L}}{N}
\end{equation}
}

\noindent holds for all $0\leq k_j\leq N$.  To prove \eqref{eq.delta_martingale}, observe that
{
\begin{align*}
&\sum_{0\leq k_{j+1}\leq N}\left(a_{j+1} + \frac{k_{j+1}l_{j+1}}{N}\right) \pi^{(N)}_{1:j+1}\left(a_1+\frac{k_1l_1}{N},\cdots, a_{j+1}+\frac{k_{j+1}l_{j+1}}{N}\right)\\
= \quad & \sum_{(t_1,\cdots, t_j)\in\left\lbrace -1, +1\right\rbrace^{j}}\int_{\prod\limits_{i=1}^jI_{i,k_i}^{(t_i)}}\prod\limits_{i=1}^jg_{i,k_i}^{(t_i)}\left[\sum_{0\leq k_{j+1}\leq N}\left(\int_{I_{j+1,k_{j+1}}^{(-1)}}g_{j+1,k_{j+1}}^{(-1)}(x_{j+1})\left(a_{j+1} + \frac{k_{j+1}l_{j+1}}{N}\right) +\right.\right.\\
& \qquad\qquad\qquad\qquad\quad\left.\left. \int_{I_{j+1,k_{j+1}}^{(+1)}}g_{j+1,k_{j+1}}^{(+1)}(x_{j+1})\left(a_{j+1} + \frac{k_{j+1}l_{j+1}}{N}\right)\right)\pi_{1:j+1}(dx_1,\cdots, dx_{j+1})\right]\\
= \quad & \sum_{(t_1,\cdots, t_j)\in\left\lbrace -1, +1\right\rbrace^{j}}\int_{\prod\limits_{i=1}^jI_{i,k_i}^{(t_i)}}\prod\limits_{i=1}^jg_{i,k_i}^{(t_i)}\left[\sum_{k_{j+1}}\int_{I_{j+1,k_{j+1}}^{(-1)}}\left(g_{j+1,k_{j+1}}^{(-1)}(x_{j+1})\left(a_{j+1} + \frac{k_{j+1}l_{j+1}}{N}\right) +\right.\right.\\
& \qquad\qquad\qquad\qquad\quad\left.\left. g_{j+1,k_{j+1}-1}^{(+1)}(x_{j+1})\left(a_{j+1} + \frac{(k_{j+1}-1)l_{j+1}}{N}\right)\right)\pi_{1:j+1}(dx_1,\cdots, dx_{j+1})\right]\\
= \quad & \sum_{(t_1,\cdots, t_j)\in\left\lbrace -1, +1\right\rbrace^{j}}\int_{\prod\limits_{i=1}^jI_{i,k_i}^{(t_i)}}\prod\limits_{i=1}^jg_{i,k_i}^{(t_i)}\left[\sum_{k_{j+1}}\int_{I_{j+1,k_{j+1}}^{(-1)}}x_{j+1}\pi_{1:j+1}(dx_1,\cdots, dx_{j+1})\right]\\
= \quad & \sum_{(t_1,\cdots, t_j)\in\left\lbrace -1, +1\right\rbrace^{j}}\int_{\prod\limits_{i=1}^jI_{i,k_i}^{(t_i)}}\prod\limits_{i=1}^jg_{i,k_i}^{(t_i)}(x_i)\left(\int_{\Omega_{j+1}}x_{j+1}\pi_{1:j+1}(dx_1,\cdots, dx_{j+1})\right)\\
\end{align*}
}
\noindent Since $\pi$ is a martingale measure, we have $\EE_{\bX\sim\pi}\left[\alpha(X_1,\cdots,X_j)(X_{j+1}-X_j)\right] = 0$ holds for all $\calF_{j}-$measurable function $\alpha$. In particular, we have
\begin{equation}
\sum_{(t_1,\cdots, t_j)\in\left\lbrace -1, +1\right\rbrace^{j}}\int_{\prod\limits_{i=1}^jI_{i,k_i}^{(t_i)}\times\Omega_{j+1}}\prod\limits_{i=1}^jg_{i,k_i}^{(t_i)}(x_i)\left(x_{j+1} - x_{j}\right)\pi_{1:j+1}(dx_1,\cdots, dx_{j+1}) = 0
\end{equation}
Hence
\begin{align*}
&\left|\sum_{0\leq k_{j+1}\leq N}\left[\left(a_{j+1} + \frac{k_{j+1}l_{j+1}}{N}\right) - \left(a_j + \frac{k_jl_j}{N}\right)\right]\pi^{(N)}_{1:j+1}\left(a_1+\frac{k_1l_1}{N},\cdots, a_{j+1}+\frac{k_{j+1}l_{j+1}}{N}\right)\right|\\
=\quad&\left|\sum_{(t_1,\cdots, t_j)\in\left\lbrace -1, +1\right\rbrace^{j}}\int_{\prod\limits_{i=1}^jI_{i,k_i}^{(t_i)}}\prod\limits_{i=1}^jg_{i,k_i}^{(t_i)}(x_i)\left(x_j- \left(a_j + \frac{k_jl_j}{N}\right)\right)\pi_{1:j}(dx_1,\cdots, dx_{j})\right|\\
\leq\quad& \frac{l_j}{N} \sum_{(t_1,\cdots, t_j)\in\left\lbrace -1, +1\right\rbrace^{j}}\int_{\prod\limits_{i=1}^jI_{i,k_i}^{(t_i)}}\prod\limits_{i=1}^jg_{i,k_i}^{(t_i)}(x_i)\pi_{1:j}(dx_1,\cdots, dx_{j})\\
\leq\quad& \frac{l_j}{N} \pi^{(N)}_{1:j}\left(a_1+\frac{k_1l_1}{N},\cdots, a_{j}+\frac{k_{j}l_{j}}{N}\right)
\end{align*}
which implies \eqref{eq.delta_martingale}.
\end{proof}

Before getting into further discussion, we impose the following seemingly strong but in fact natural  technical assumption on the support of marginals.
\begin{assumption}\label{aspn.disperse}
\[
\tau := \min_{1\leq i\leq d-1}\left\lbrace a_i - a_{i+1}\right\rbrace\wedge\min_{1\leq i\leq d-1}\left\lbrace b_{i+1} - b_i\right\rbrace >0
\]
i.e, the support of marginals become more and more dispersed over time.
\end{assumption}
Let $\calM\left(\Pi_{i=1}^d\Omega^{(N)}_i;\delta\right)$ be the set of all the $\delta-$martingale measures  that supported on $\Pi_{i=1}^d\Omega^{(N)}_i$, now we define 
\begin{equation}
I_{\left(\widehat{\mu}_1^{(n)},\widehat{\mu}_2^{(n)},\cdots,\widehat{\mu}_d^{(n)}\right)}^{(N)}(f; \varepsilon, \delta)  := 
\sup_{\pi\in\calP^{(N)}_{\left(\widehat{\mu}_1^{(n)},\widehat{\mu}_2^{(n)},\cdots,\widehat{\mu}_d^{(n)}\right)}(\varepsilon,\delta)}\EE_{\pi}\left[f(X_1,\cdots,X_d)\right]
\end{equation}
where 
\begin{equation}
\calP^{(N)}_{\left(\widehat{\mu}_1^{(n)},\widehat{\mu}_2^{(n)},\cdots,\widehat{\mu}_d^{(n)}\right)}( \varepsilon, 
\delta) := \left\lbrace \pi\in\calM\left(\Pi_{i=1}^d\Omega^{(N)}_i;\delta\right):  \sum_{i=1}^d\calW(
\widehat{\mu}_i^{(n)},\pi_i)<\varepsilon\right\rbrace
\end{equation}
It is easy to see that $I^{(N)}_{\left(\widehat{\mu}_1^{(n)},\widehat{\mu}_2^{(n)},\cdots,\widehat{\mu}_d^{(n)}\right)}(f; \varepsilon,\delta) $ is essentially a finite dimensional LP, which can be solved by generic LP Algorithm. 
The following concentration result shows that this is a good estimator (picking $\delta \asymp 1/N$) for $I_{\left(\widehat{\mu}_1^{(n)},\widehat{\mu}_2^{(n)},\cdots,\widehat{\mu}_d^{(n)}\right)}(f; \varepsilon) $ when $N$ sufficiently large.
\begin{theorem}\label{thm.discretize_approximation}
Given $\varepsilon >0$, $\delta\in(0,1)$, with probability at least $1-\delta$ we have
\begin{equation}\label{eq.discretize_approximation}
\left|I_{\left(\widehat{\mu}_1^{(n)},\widehat{\mu}_2^{(n)},\cdots,\widehat{\mu}_d^{(n)}\right)}(f; \varepsilon) - I^{(N)}_{\left(\widehat{\mu}_1^{(n)},\widehat{\mu}_2^{(n)},\cdots,\widehat{\mu}_d^{(n)}\right)}\left(f; \varepsilon + \frac{\widetilde{L}d^{3/2}}{N},  \frac{\widetilde{L}}{N}\right)\right|\leq\frac{C(f,\varepsilon, d, \Omega)}{N}
\end{equation}
holds when $n\geq N(\varepsilon,\delta) = \frac{d^2}{C_2}\log\left(\frac{dC_1}{\delta}\right)\varepsilon^{-2}$, where $C(f,\varepsilon, d, \Omega)$ is a constant depends on $f,\varepsilon, d$ and $\Omega$
\end{theorem}

\begin{proof}
We first show that  $\calP^{(N)}_{\left(\widehat{\mu}_1^{(n)},\widehat{\mu}_2^{(n)},\cdots,\widehat{\mu}_d^{(n)}\right)}\left(\varepsilon + \frac{Cd^{3/2}\widetilde{L}}{N}; \frac{\widetilde{L}}{N}\right)\neq \varnothing$ with probability at least $1-\delta$ for $n\geq N(\varepsilon,\delta)$, which ensure the optimization problems in LHS of \eqref{eq.discretize_approximation} are feasible. 

For any $\pi \in\calP_{\left(\widehat{\mu}_1^{(n)},\widehat{\mu}_2^{(n)},\cdots,\widehat{\mu}_d^{(n)}\right)}(\varepsilon)$, by Lemma \ref{lemma.discretize} there exists a $\widetilde{L}/N-$martingale measure $\pi'\in\calP\left(\Pi_{i=1}^d\Omega^{(N)}_i\right)$ with $\calW(\pi',\pi)\leq\frac{\widetilde{L}\sqrt{d}}{N}$, and consequently $$\sum_{i=1}^d\calW\left(\pi_i',\widehat{\mu}_i^{(n)}\right)\leq\sum_{i=1}^d\calW\left(\pi_i,\widehat{\mu}_i^{(n)}\right) + \sum_{i=1}^d\calW(\pi'_i,\pi_i)\leq \varepsilon + \sum_{i=1}^d\calW(\pi',\pi) \leq \varepsilon + \frac{\widetilde{L}d^{3/2}}{N}$$
In other words, we have $\pi'\in\calP^{(N)}_{\left(\widehat{\mu}_1^{(n)},\widehat{\mu}_2^{(n)},\cdots,\widehat{\mu}_d^{(n)}\right)}\left(\varepsilon + \frac{d^{3/2}\widetilde{L}}{N}; \frac{\widetilde{L}}{N}\right)\neq\varnothing$. Furthermore, 
\begin{equation}
\begin{aligned}
\EE_{\bX\sim\pi}f(\bX) - I^{(N)}_{\left(\widehat{\mu}_1^{(n)},\widehat{\mu}_2^{(n)},\cdots,\widehat{\mu}_d^{(n)}\right)}\left(f; \varepsilon + \frac{\widetilde{L}d^{3/2}}{N},  \frac{\widetilde{L}}{N}\right) &\leq \EE_{\bX\sim\pi}f(\bX) - \EE_{\bX\sim\pi'}f(\bX) \\
&\leq L \calW(\pi',\pi)\leq\frac{\widetilde{L}L\sqrt{d}}{N}
\end{aligned}
\end{equation}
Taking the supremum over $\pi \in\calP_{\left(\widehat{\mu}_1^{(n)},\widehat{\mu}_2^{(n)},\cdots,\widehat{\mu}_d^{(n)}\right)}(\varepsilon)$ yields
\begin{equation}\label{eq.RHS_discretize_approximation}
I_{\left(\widehat{\mu}_1^{(n)},\widehat{\mu}_2^{(n)},\cdots,\widehat{\mu}_d^{(n)}\right)}(f; \varepsilon) -  I^{(N)}_{\left(\widehat{\mu}_1^{(n)},\widehat{\mu}_2^{(n)},\cdots,\widehat{\mu}_d^{(n)}\right)}\left(f; \varepsilon + \frac{\widetilde{L}d^{3/2}}{N},  \frac{\widetilde{L}}{N}\right)  \leq \frac{\widetilde{L}L\sqrt{d}}{N}
\end{equation}
Next we lower bounded the LHS of \eqref{eq.RHS_discretize_approximation}. Recalled from Corollary \ref{cor.dual_reformulation} and Theorem \ref{thm.distance_n} that
\begin{equation}
I_{\left(\widehat{\mu}_1^{(n)},\widehat{\mu}_2^{(n)},\cdots,\widehat{\mu}_d^{(n)}\right)}(f; \varepsilon) = 
\inf_{\mbox{$\begin{subarray}{c} \widetilde\calS_{\left(\widehat{\mu}_1^{(n)},\widehat{\mu}_2^{(n)},\cdots,\widehat{\mu}_d^{(n)}\right)}(\varepsilon),\\
\gamma \leq \frac{4}{\varepsilon}\sup_{\bX\in\Omega}f(\bX)\end{subarray}$}}\gamma\varepsilon + \int_{\Omega_d}
F\left(x_d\right)\widehat{\mu}_d^{(n)}(dx_d)
\end{equation}
holds with probability at least $1-\delta$ for $n\geq N\left(\varepsilon/2, \delta \right)$, where $F(x_d)$ is an abbreviation of 
\begin{equation}\label{eq.thm.discretize_F(x_d)}
\begin{aligned}
F\left(x_d; \gamma, \left\lbrace\alpha_k\right\rbrace_{k=1}^{d-1}, \left\lbrace\beta_k\right\rbrace_{k=1}^{d-1}\right)  : = \sup_{\mbox{$\begin{subarray}{c} x_k\in\Omega_k, 1\leq k\leq d-1,\\
x_k'\in\Omega_k, 1\leq k\leq d\end{subarray}$}}\left\lbrace f\left(\bX'\right)- \sum_{k=1}^{d-1}\beta_k(x_k)-\gamma\sum_{k=1}^{d}|x_k-x_k'| + \sum_{k=1}^{d-1}\alpha_k(\bX_k')(x_{k+1}'-x_k')\right\rbrace
\end{aligned}
\end{equation}
Note that 
\begin{align*}
F(x_d)&\geq \sup_{\mbox{$\begin{subarray}{c} x_k\in\Omega_k, 1\leq k\leq d-1,\\
x_k'\in\Omega_k, 1\leq k\leq d\end{subarray}$}}\left\lbrace f\left(\bX'\right)- \sum_{k=1}^{d-1}\beta_k(x_k)+ \sum_{k=1}^{d-1}\alpha_k(\bX_k')(x_{k+1}'-x_k')\right\rbrace - \gamma \sum_{i=1}^dl_i\\
&= \sup_{x_k'\in\Omega_k, 1\leq k\leq d}\left\lbrace  \sum_{k=1}^{d-1}\alpha_k(\bX_k')(x_{k+1}'-x_k')\right\rbrace + \inf_{\bX'\in\Omega}f\left(\bX'\right) - \sum_{k=1}^{d-1}\inf_{x_k\in\Omega_k}\beta_k(x_k) - \gamma d\widetilde{L}\\
&\geq \sup_{x_k'\in\Omega_k, 1\leq k\leq d}\left\lbrace  \sum_{k=1}^{d-1}\alpha_k(\bX_k')(x_{k+1}'-x_k')\right\rbrace + \inf_{\bX'\in\Omega}f\left(\bX'\right) - \gamma d\widetilde{L}
\end{align*}
In the last step we've used the fact that  $\inf_{x_k\in\Omega_k}\beta_k(x_k)\leq\int_{\Omega_k}\beta_k(x_k)\mu_k(dx_k) = 0$ $(k=1,2,\cdots,d-1)$ for $\beta_{k}$'s in $\widetilde\calS_{\left(\widehat{\mu}_1^{(n)},\widehat{\mu}_2^{(n)},\cdots,\widehat{\mu}_d^{(n)}\right)}(\varepsilon)$. By letting $x_i' = x_2'$ for all $2\leq i\leq d$, we have 
\begin{align*}
F(x_d)\geq \sup_{x_1'\in\Omega_1, x_2'\in\Omega_2}\left\lbrace \alpha_1(x_1')(x_2' - x_1')\right\rbrace +  \inf_{\bX'\in\Omega}f\left(\bX'\right) - \gamma d\widetilde{L}
\end{align*}
Suppose $\|\alpha_1\|_{\infty}:=\sup_{x_1'\in\Omega_1}|\alpha_1(x_1')|> B_1$ for some positive number $B_1$. If there exists an $x_1^*\in\Omega_1$ such that $\alpha_1(x_1^*)\geq B_1$, by Assumption \ref{aspn.disperse} we get
\begin{equation}
F(x_d)\geq \alpha_1(x_1^*)(b_2 - x_1^*) + \inf_{\bX'\in\Omega}f\left(\bX'\right) - \gamma d\widetilde{L}> \tau B_1 + \inf_{\bX'\in\Omega}f\left(\bX'\right) - \gamma d\widetilde{L}
\end{equation}
Similarily, if there exits an $x_1^*\in\Omega_1$ such that $\alpha_1(x_1^*)\leq -B_1$, then 
\begin{equation}
F(x_d)\geq \alpha_1(x_1^*)(a_2 - x_1^*) + \inf_{\bX'\in\Omega}f\left(\bX'\right) - \gamma d\widetilde{L}> \tau B_1+ \inf_{\bX'\in\Omega}f\left(\bX'\right) - \gamma d\widetilde{L}
\end{equation}
Combining with the bound of $\gamma$ shown in Theorem \ref{thm.distance_n}, we have
\begin{align*}
\inf_{\mbox{$\begin{subarray}{c} \widetilde\calS_{\left(\widehat{\mu}_1^{(n)},\widehat{\mu}_2^{(n)},\cdots,\widehat{\mu}_d^{(n)}\right)}(\varepsilon),\\
\|\alpha_1\|_{\infty}> B_1, \gamma \leq \frac{4}{\varepsilon}\sup_{\bX\in\Omega}f(\bX)\end{subarray}$}}\gamma\varepsilon + \int_{\Omega_d}
F\left(x_d\right)\widehat{\mu}_d^{(n)}(dx_d) &\geq \gamma\varepsilon + \int_{\Omega_d}\left[\tau B_1+ \inf_{\bX'\in\Omega}f\left(\bX'\right) - \gamma d\widetilde{L}\right]\widehat{\mu}_d^{(n)}(dx_d)\\
&\geq \tau B_1+ \inf_{\bX'\in\Omega}f\left(\bX'\right) -  \frac{4}{\varepsilon}\sup_{\bX\in\Omega}f(\bX)d\widetilde{L}\\
&> \sup_{\bX\in\Omega}f(\bX)\\
&\geq I_{\left(\widehat{\mu}_1^{(n)},\widehat{\mu}_2^{(n)},\cdots,\widehat{\mu}_d^{(n)}\right)}(f; \varepsilon) 
\end{align*}
where we've set $B_1 = \frac{\left[\frac{4d\widetilde{L}}{\varepsilon} + 2\right]\sup_{\bX\in\Omega}|f(\bX)|}{\tau}$. 
As a result,
\begin{equation}
I_{\left(\widehat{\mu}_1^{(n)},\widehat{\mu}_2^{(n)},\cdots,\widehat{\mu}_d^{(n)}\right)}(f; \varepsilon) = \inf_{\mbox{$\begin{subarray}{c} \widetilde\calS_{\left(\widehat{\mu}_1^{(n)},\widehat{\mu}_2^{(n)},\cdots,\widehat{\mu}_d^{(n)}\right)}(\varepsilon),\\
\|\alpha_1\|_{\infty}\leq B_1, \gamma \leq \frac{4}{\varepsilon}\sup_{\bX\in\Omega}f(\bX)\end{subarray}$}}\gamma\varepsilon + \int_{\Omega_d}
F\left(x_d\right)\widehat{\mu}_d^{(n)}(dx_d)
\end{equation}
Next we use induction argument to show that indeed each $\alpha_i$ has bounded supremum norm. Suppose we have 
\begin{equation}
I_{\left(\widehat{\mu}_1^{(n)},\widehat{\mu}_2^{(n)},\cdots,\widehat{\mu}_d^{(n)}\right)}(f; \varepsilon) = \inf_{\mbox{$\begin{subarray}{c} \widetilde\calS_{\left(\widehat{\mu}_1^{(n)},\widehat{\mu}_2^{(n)},\cdots,\widehat{\mu}_d^{(n)}\right)}(\varepsilon),\\
\|\alpha_i\|_{\infty}\leq B_i, 1\leq i\leq m, \gamma \leq \frac{4}{\varepsilon}\sup_{\bX\in\Omega}f(\bX)\end{subarray}$}}\gamma\varepsilon + \int_{\Omega_d}
F\left(x_d\right)\widehat{\mu}_d^{(n)}(dx_d)
\end{equation}
for some $1\leq m\leq d-2$. Conditioning on  $\gamma \leq \frac{4}{\varepsilon}\sup_{\bX\in\Omega}|f(\bX)|$ and $\|\alpha_i\|_{\infty}\leq B_i, 1\leq i\leq m$, we have 
\begin{align*}
F(x_d)&\geq \sup_{x_k'\in\Omega_k, 1\leq k\leq d}\left\lbrace  \sum_{k=1}^{d-1}\alpha_k(\bX_k')(x_{k+1}'-x_k')\right\rbrace + \inf_{\bX'\in\Omega}f\left(\bX'\right) - \gamma d\widetilde{L}\\
&\geq \sup_{x_k'\in\Omega_k, m+1\leq k\leq d}\left\lbrace \sum_{k=m+1}^{d-1}\alpha_k(\bX_k')(x_{k+1}'-x_k')\right\rbrace -\sum_{k=1}^m B_il_i + \inf_{\bX'\in\Omega}f\left(\bX'\right) - \gamma d\widetilde{L}
\end{align*}
Now taking $x_k' = x_{m+2}$ for all $k\geq m+2$, and by similar argument in bounding $\|\alpha_1\|_{\infty}$, conditioning on $\|\alpha_{m+1}\|_{\infty}> B_{m+1}$, we can lower bounded $F(x_d)$ by 
\begin{align*}
F(x_d)&\geq \sup_{x_{m+1}'\in\Omega_{m+1}, x_{m+2}'\in\Omega_{m+2}}\left\lbrace \alpha_{m+1}\left(\bX'_{m+1}\right)(x'_{m+2}-x'_{m+1})\right\rbrace - \widetilde{L}\sum_{k=1}^mB_i+\inf_{\bX'\in\Omega}f\left(\bX'\right) - \gamma d\widetilde{L}\\
&\geq \inf_{\bX'\in\Omega}f\left(\bX'\right) - \frac{4}{\varepsilon}\sup_{\bX\in\Omega}f(\bX) d\widetilde{L} + \tau B_{m+1}  - \widetilde{L}\sum_{k=1}^mB_i
\end{align*}
Hence
{\small
\begin{align*}
\inf_{\mbox{$\begin{subarray}{c} \widetilde\calS_{\left(\widehat{\mu}_1^{(n)},\widehat{\mu}_2^{(n)},\cdots,\widehat{\mu}_d^{(n)}\right)}(\varepsilon),\\
\|\alpha_i\|_{\infty}\leq B_i, 1\leq i\leq m, \|\alpha_{m+1}\|_{\infty}> B_{m+1},\\
\gamma \leq \frac{4}{\varepsilon}\sup_{\bX\in\Omega}f(\bX) \end{subarray}$}}\gamma\varepsilon + \int_{\Omega_d}
F\left(x_d\right)\widehat{\mu}_d^{(n)}(dx_d) &\geq  \inf_{\bX'\in\Omega}f\left(\bX'\right) - \frac{4}{\varepsilon}\sup_{\bX\in\Omega}f(\bX) d\widetilde{L} + \tau B_{m+1}  - \widetilde{L}\sum_{k=1}^mB_i\\
&> \sup_{\bX\in\Omega}f(\bX)\geq I_{\left(\widehat{\mu}_1^{(n)},\widehat{\mu}_2^{(n)},\cdots,\widehat{\mu}_d^{(n)}\right)}(f; \varepsilon) 
\end{align*}
}
where 
\begin{equation}\label{eq.iteration_Bi}
B_{m+1}:= \frac{\left[\frac{4d\widetilde{L}}{\varepsilon} + 2\right]\sup_{\bX\in\Omega}|f(\bX)|}{\tau}+\frac{\widetilde{L}}{\tau}\sum_{k=1}^mB_k = B_1 + \frac{\widetilde{L}}{\tau}\sum_{k=1}^mB_k
\end{equation}
Now we come to the following result, 
\begin{equation}
I_{\left(\widehat{\mu}_1^{(n)},\widehat{\mu}_2^{(n)},\cdots,\widehat{\mu}_d^{(n)}\right)}(f; \varepsilon) = \inf_{\mbox{$\begin{subarray}{c} \widetilde\calS_{\left(\widehat{\mu}_1^{(n)},\widehat{\mu}_2^{(n)},\cdots,\widehat{\mu}_d^{(n)}\right)}(\varepsilon),\\
\|\alpha_i\|_{\infty}\leq B_i, 1\leq i\leq m+1, 0\leq\gamma \leq \frac{4}{\varepsilon}\sup_{\bX\in\Omega}|f(\bX)|\end{subarray}$}}\gamma\varepsilon + \int_{\Omega_d}
F\left(x_d\right)\widehat{\mu}_d^{(n)}(dx_d)
\end{equation}
which complete the induction. Moreover, note that \eqref{eq.iteration_Bi} holds for all $1\leq m\leq d-1$, we have $B_{m}\leq \left(1+\frac{\widetilde{L}}{\tau}\right)^{m-1}B_1$ via a simple induction argument. Now we are able to give a lower bound of the LHS of \eqref{eq.RHS_discretize_approximation}. Follows the directly from Theorme \ref{thm.strongdual}, one can show the strong duality also holds for  $I_{\left(\widehat{\mu}_1^{(n)},\widehat{\mu}_2^{(n)},\cdots,\widehat{\mu}_d^{(n)}\right)}\left(f; \varepsilon + \frac{\widetilde{L}d^{3/2}}{N},  \frac{\widetilde{L}}{N}\right)$. We omit the detailed proof and state the result as following
\begin{equation}
I_{\left(\widehat{\mu}_1^{(n)},\widehat{\mu}_2^{(n)},\cdots,\widehat{\mu}_d^{(n)}\right)}\left(f; \varepsilon + \frac{\widetilde{L}d^{3/2}}{N},  \frac{\widetilde{L}}{N}\right) = \inf_{ \widetilde\calS_{\left(\widehat{\mu}_1^{(n)},\widehat{\mu}_2^{(n)},\cdots,\widehat{\mu}_d^{(n)}\right)}(\varepsilon)}\gamma\left(\varepsilon + \frac{\widetilde{L}d^{3/2}}{N}\right)+ \int_{\Omega_d}
\widetilde{F}\left(x_d\right)\widehat{\mu}_d^{(n)}(dx_d)
\end{equation}
where 
\begin{equation}
\begin{aligned}
\widetilde{F}\left(x_d\right) : = \sup_{\mbox{$\begin{subarray}{c} x_k\in\Omega_k, 1\leq k\leq d-1,\\
x_k'\in\Omega_k, 1\leq k\leq d\end{subarray}$}}\left\lbrace f\left(\bX'\right) + \sum_{k=1}^{d-1}\frac{\widetilde{L}}{N}|\alpha_k(\bX'_k)| + \sum_{k=1}^{d-1}\alpha_k(\bX_k')(x_{k+1}'-x_k') \right.\\
\left. + \sum_{k=1}^{d-1}\beta_k(x_k)-\gamma\sum_{k=1}^{d}|x_k-x_k'| \right\rbrace
\end{aligned}
\end{equation}
\noindent For any $\Delta >0$, we can pick $$\left(\gamma_{\Delta}, \left\lbrace\alpha_{k,\Delta}\right\rbrace_{k=1}^{d-1}, \left\lbrace\beta_{k,\Delta}\right\rbrace_{k=1}^{d-1}\right)\in\widetilde\calS_{\left(\widehat{\mu}_1^{(n)},\widehat{\mu}_2^{(n)},\cdots,\widehat{\mu}_d^{(n)}\right)}(\varepsilon)\cap\left\lbrace \|\alpha_i\|_{\infty}\leq B_i, 1\leq i\leq d-1, \gamma \leq \frac{4}{\varepsilon}\sup_{\bX\in\Omega}f(\bX) \right\rbrace$$ such that 
\begin{equation*}
\gamma_{\Delta}\varepsilon + \int_{\Omega_d}
F_{\Delta}\left(x_d\right)\widehat\mu_d^{(n)}(dx_d)\leq I_{\left(\widehat{\mu}_1^{(n)},\widehat{\mu}_2^{(n)},\cdots,\widehat{\mu}_d^{(n)}\right)}(f; \varepsilon)  + \Delta
\end{equation*}
where $F_{\Delta}(x_d)$ denotes the value of $F(x_d)$ after plugging $\left(\gamma_{\Delta}, \left\lbrace\alpha_{k,\Delta}\right\rbrace_{k=1}^{d-1}, \left\lbrace\beta_{k,\Delta}\right\rbrace_{k=1}^{d-1}\right)$ in \eqref{eq.thm.discretize_F(x_d)}, similarily we can define $\widetilde{F}_{\Delta}(x_d)$. Hence 
\begin{align*}
& I^{(N)}_{\left(\widehat{\mu}_1^{(n)},\widehat{\mu}_2^{(n)},\cdots,\widehat{\mu}_d^{(n)}\right)}\left(f; \varepsilon + \frac{\widetilde{L}d^{3/2}}{N},  \frac{\widetilde{L}}{N}\right)  - I_{\left(\widehat{\mu}_1^{(n)},\widehat{\mu}_2^{(n)},\cdots,\widehat{\mu}_d^{(n)}\right)}(f; \varepsilon)\\
\leq \quad &I_{\left(\widehat{\mu}_1^{(n)},\widehat{\mu}_2^{(n)},\cdots,\widehat{\mu}_d^{(n)}\right)}\left(f; \varepsilon + \frac{\widetilde{L}d^{3/2}}{N},  \frac{\widetilde{L}}{N}\right)  - I_{\left(\widehat{\mu}_1^{(n)},\widehat{\mu}_2^{(n)},\cdots,\widehat{\mu}_d^{(n)}\right)}(f; \varepsilon) \\
\leq \quad& \gamma_{\Delta}\left(\varepsilon + \frac{\widetilde{L}d^{3/2}}{N}\right)+ \int_{\Omega_d} \widetilde{F}_{\Delta}(x_d)\widehat{\mu}_d^{(n)}(dx_d) - \left(\gamma_{\Delta}\varepsilon + \int_{\Omega_d}
F_{\Delta}\left(x_d\right)\widehat{\mu}_d^{(n)}(dx_d)\right) + \Delta\\
\leq \quad& \frac{4}{\varepsilon}\sup_{\bX\in\Omega}|f(\bX)|\cdot \frac{\widetilde{L}d^{3/2}}{N} + \int_{\Omega_d}\left(\widetilde{F}_{\Delta}(x_d) - F_{\Delta}(x_d)\right)\widehat{\mu}_d^{(n)}(dx_d) + \Delta\\
\leq \quad& \frac{4}{\varepsilon}\sup_{\bX\in\Omega}|f(\bX)|\cdot \frac{\widetilde{L}d^{3/2}}{N} + \frac{\widetilde{L}}{N}\sum_{i=1}^{d-1}B_i + \Delta\\
\leq \quad& \frac{1}{N}\left[\frac{4\widetilde{L}d^{3/2}}{\varepsilon}\sup_{\bX\in\Omega}|f(\bX)| + \left(1+\frac{\widetilde{L}}{\tau}\right)^{d-1}\left(\frac{4d\widetilde{L}}{\varepsilon} + 2\right)\sup_{\bX\in\Omega}|f(\bX)|\right] + \Delta
\end{align*}
Letting $\Delta\rightarrow 0$, and combining with \eqref{eq.RHS_discretize_approximation}, we have
\begin{equation}
\left|I_{\left(\widehat{\mu}_1^{(n)},\widehat{\mu}_2^{(n)},\cdots,\widehat{\mu}_d^{(n)}\right)}(f; \varepsilon) - I^{(N)}_{\left(\widehat{\mu}_1^{(n)},\widehat{\mu}_2^{(n)},\cdots,\widehat{\mu}_d^{(n)}\right)}\left(f; \varepsilon + \frac{\widetilde{L}d^{3/2}}{N},  \frac{\widetilde{L}}{N}\right)\right|\leq\frac{C(f,\varepsilon, d, \Omega)}{N}
\end{equation}
where $$C(f,\varepsilon, d, \Omega):= \max\left\lbrace \left[\frac{4\widetilde{L}d^{3/2}}{\varepsilon} + \left(1+\frac{\widetilde{L}}{\tau}\right)^{d-1}\left(\frac{4d\widetilde{L}}{\varepsilon} + 2\right)\right]\sup_{\bX\in\Omega}|f(\bX)|, \widetilde{L}L\sqrt{d}\right\rbrace$$ is a constant only depends on $f,\varepsilon, d$ and $\Omega$.
\end{proof}

==> defs.tex <==
\newcommand{\ones}{\mathbf 1}
\newcommand{\reals}{{\mbox{\bf R}}}
\newcommand{\integers}{{\mbox{\bf Z}}}
\newcommand{\symm}{{\mbox{\bf S}}}  % symmetric matrices

\newcommand{\nullspace}{{\mathcal N}}
\newcommand{\range}{{\mathcal R}}
\newcommand{\Rank}{\mathop{\bf Rank}}
\newcommand{\Tr}{\mathop{\bf Tr}}
\newcommand{\diag}{\mathop{\bf diag}}
\newcommand{\card}{\mathop{\bf card}}
\newcommand{\rank}{\mathop{\bf rank}}
\newcommand{\conv}{\mathop{\bf conv}}
\newcommand{\prox}{\mathbf{prox}}

\newcommand{\Expect}{\mathop{\bf E{}}}
\newcommand{\Prob}{\mathop{\bf Prob}}
\newcommand{\Co}{{\mathop {\bf Co}}} % convex hull
\newcommand{\dist}{\mathop{\bf dist{}}}
\newcommand{\argmin}{\mathop{\rm argmin}}
\newcommand{\argmax}{\mathop{\rm argmax}}
\newcommand{\epi}{\mathop{\bf epi}} % epigraph
\newcommand{\Vol}{\mathop{\bf vol}}
\newcommand{\dom}{\mathop{\bf dom}} % domain
\newcommand{\intr}{\mathop{\bf int}}
\newcommand{\sign}{\mathop{\bf sign}}

\newcommand{\cf}{{\it cf.}}
\newcommand{\eg}{{\it e.g.}}
\newcommand{\ie}{{\it i.e.}}
\newcommand{\etc}{{\it etc.}}


==> dual.tex <==
The following strong duality theorem for the distributionally robust worst-case expectation with martingale constraint is a key step when proving the concentration result.

\begin{theorem} \label{thm.strongdual}
Under Assumption \ref{aspn.compact_support}, suppose we have $\calP_{(\nu_1,\nu_2,\cdots,\nu_d)}(\varepsilon)\ne\varnothing$ for some $\varepsilon>0$ and probability measures $\nu_i\in\calP(\Omega_i)$, $i=1,2,\cdots, d$, then the dual representation of 
\begin{equation}
I_{(\nu_1,\cdots,\nu_d)}(f;\varepsilon) := 
\sup_{\pi\in\calP_{(\nu_1,\nu_2,\cdots,\nu_d)}(\varepsilon)}\EE_{\bX\sim \pi}\left[f(\mathbf{X})\right].
\end{equation}	
 is the following:
\begin{align*}
J_{(\nu_1,\cdots,\nu_d)}(f;\varepsilon)  := \emph{inf} \quad &  \gamma\varepsilon + \sum_{k=1}^d\int_{\Omega_k}\beta_k(x_k)\nu_k(dx_k)\\
\emph{subject to} \quad & \gamma\geq 0; \\ & \alpha_k(x_1',\cdots,x_k')\in C\left(\Omega_1\times\cdots\times\Omega_k\right), 1\leq k\leq d-1; \\
& \beta_k(x_k)\in C(\Omega_k), 1\leq k\leq d;\\
& f(x_1',\cdots, x_d') + \sum_{k=1}^{d-1}\alpha_k(x_1',\cdots, x_k')(x_{k+1}' - x_k')-\gamma\sum_{k=1}^d|x_k-x_k'|\\
&-\sum_{k=1}^{d}\beta_k(x_k)\leq 0, \quad \forall x_k, x_k' \in \Omega_k.
\end{align*} 
Moreover, we have the following strong duality 
\[
I_{(\nu_1,\cdots,\nu_d)}(f;\varepsilon) = J_{(\nu_1,\cdots,\nu_d)}(f;\varepsilon).
\]
and there exist a primal optimizer $\pi^*\in\calP_{(\nu_1,\nu_2,\cdots,\nu_d)}(\varepsilon)$ for $I_{(\nu_1,\cdots,\nu_d)}(f;\varepsilon)$. 
\end{theorem}
We invoke the following min-max theorem of decision theory by Sion to prove the Theorem \ref{thm.strongdual}.

\begin{lemma} [Sion's minimax theorem, \cite{sion1958general}] \label{sion}
Let $X$ be a compact convex subset of a linear topological space and $Y$ a convex subset of a linear topological space. If $f$ is a real-valued function on $X\times Y$ with
\begin{enumerate}
\item [\emph{(1)}] $f(x,\cdot)$ lower semi-continuous and quasi-convex on $Y$, $\forall x\in X$.
\item [\emph(2)] $f(\cdot,y)$ upper semi-continuous and quasi-concave on $X$, $\forall y\in Y$.
\end{enumerate}
then,
\[
\max _{x\in X}\inf _{y\in Y}f(x,y)=\inf _{y\in Y}\max _{x\in X}f(x,y)
\]
\end{lemma}

\begin{proof}[Proof of Theorem \ref{thm.strongdual}]
Note that weak duality $I_{(\nu_1,\cdots,\nu_d)}(\varepsilon)\leq J_{(\nu_1,\cdots,\nu_d)}(\varepsilon)$ always hold, to proof the desired strong duality we just need to show the reverse inequality also hold. 

Define $\bX = (x_1,\cdots, x_d)$ and $\bX' = (x_1',\cdots, x_d')$. Consider the following function
\begin{align*}
\calL\left(\bpi,\gamma,\left\lbrace\alpha_k\right\rbrace_{k=1}^{d-1}, \left\lbrace\beta_k\right\rbrace_{k=1}^{d} \right) &=\int_{\Omega\times\Omega} \left[f\left(\bX'\right)+\sum_{k=1}^{d-1}\alpha_k(x_1',\cdots,x_k')(x_{k+1}'-x_k')-\sum_{k=1}^{d}\beta_k(x_k)\right]\bpi(d\bX, d\bX') \\
&\qquad +\gamma\left(\varepsilon - \int_{\Omega\times\Omega} \sum_{k=1}^d|x_k-x_k'| \bpi(d\bX, d\bX')\right) + \sum_{k=1}^d\int_{\Omega_k}\beta_k(x_k)\nu_k(dx_k)
\end{align*}
with
\begin{align*}
&\alpha_k(x_1',\cdots,x_k')\in C\left(\Omega_1\times\cdots\times\Omega_k\right), 1\leq k\leq d-1;\quad \beta_k(x_k)\in C(\Omega_k), 1\leq k\leq d; \quad \gamma \ge 0,\\
&\bpi \in \bPi \triangleq \{\text{Borel probability measures on $\Omega\times\Omega$}\}. 
\end{align*}
Note that by Assumption \ref{aspn.compact_support}  we have $\Omega:=\Omega_1\times\cdots\times\Omega_d$ is a compact subset of $\RR^d$, thus $\Omega\times\Omega$ endowed with the usual metric is a compact Polish Space. As a result, we have $\bPi$ is compact with respect to the weak topology. Moreover, since $f, \left\lbrace\alpha_k\right\rbrace_{k=1}^{d-1}, \left\lbrace\beta_k\right\rbrace_{k=1}^{d}$ are continuous functions and the support of $\bpi$ is bounded, we have $\calL$ is continuous in $\bpi$.
Finally, equip each $C(\Omega_1\times\cdots\times\Omega_k)$ ($1\leq k\leq d-1$), $C(\Omega_k)$ ($1\leq k\leq d$) the uniform (with sup-norm) topology and $\gamma\in \RR_{\geq0}$ the Euclidean topology, we have that $\calL$ is also continuous in $\gamma$, $\alpha_k$ ($1\leq k\leq d-1$) and $\beta_k$ ($1\leq k\leq d$). Finally, $\calL$ is affine in $\left(\pi,\gamma,\left\lbrace\alpha_k\right\rbrace_{k=1}^{d-1}, \left\lbrace\beta_k\right\rbrace_{k=1}^{d}\right)$, now we can invoke the Sion's minimax theorem (Lemma \ref{sion}) to obtain

\begin{align}\label{eq.sion-minimax}
\sup_{\bpi \in \bPi} \inf_{\mbox{$\begin{subarray}{c}\{\alpha_k\in C(\Omega_1\times\cdots\times\Omega_k)\}_{k=1}^{d-1}\\
\{\beta_k\in C(\Omega_k)\}_{k=1}^{d}\\		
\gamma\ge 0\end{subarray}$}} \calL\left(\bpi,\gamma,\left\lbrace\alpha_k\right\rbrace_{k=1}^{d-1}, \left\lbrace\beta_k\right\rbrace_{k=1}^{d}\right) =  \inf_{\mbox{$\begin{subarray}{c}\{\alpha_k\in C(\Omega_1\times\cdots\times\Omega_k)\}_{k=1}^{d-1}\\
\{\beta_k\in C(\Omega_k)\}_{k=1}^{d}\\		
\gamma\ge 0\end{subarray}$}}\sup_{\bpi \in \bPi} \calL\left(\bpi,\gamma,\left\lbrace\alpha_k\right\rbrace_{k=1}^{d-1}, \left\lbrace\beta_k\right\rbrace_{k=1}^{d}\right)
\end{align}
Let $\pi$ be the maringal of $\bpi$ on $\bX'$, we can rewrite the function $\calL$ by
\begin{align*}
\calL\left(\bpi,\gamma,\left\lbrace\alpha_k\right\rbrace_{k=1}^{d-1}, \left\lbrace\beta_k\right\rbrace_{k=1}^{d} \right) &=\EE_{\bX'\sim\pi}f(\bX') +  \int_{\Omega} \left[\sum_{k=1}^{d-1}\alpha_k(x_1',\cdots,x_k')(x_{k+1}'-x_k')\right]\pi(d\bX') \\
&+ \sum_{k=1}^d\left[\int_{\Omega_k}\beta_k(x_k)\nu_k(dx_k) - \int_{\Omega}\beta_k(x_k)\bpi(d\bX,d\bX')\right]\\
&+\gamma\left(\varepsilon - \int_{\Omega\times\Omega} \sum_{k=1}^d|x_k-x_k'| \bpi(d\bX, d\bX')\right) 
\end{align*}
Given any feasible $\bpi\in\bPi$, consider the inner infimum of the LHS in \eqref{eq.sion-minimax}, prevent it from being $-\infty$ we have 
\begin{equation}{\label{mart_alpha}}
\int_{\Omega} \alpha_k(x_1',\cdots,x_k')(x_{k+1}'-x_k')\pi(d\bX') = 0, \qquad  \forall \alpha_k\in C(\Omega_1\times\cdots\times\Omega_k), \quad \forall1\leq k\leq d-1.
\end{equation}
\begin{equation}\label{margin_beta}
\int_{\Omega_k}\beta_k(x_k)\nu_k(dx_k) - \int_{\Omega}\beta_k(x_k)\bpi(d\bX,d\bX') = 0, \quad \beta_k(x_k)\in C(\Omega_k), \quad \forall 1\leq k\leq d
\end{equation}
and 
\begin{equation}\label{robust_gamma}
\int_{\Omega\times\Omega} \sum_{k=1}^d|x_k-x_k'| \bpi(d\bX, d\bX')\leq \varepsilon
\end{equation}
Let $\calF_k'=\sigma\left(X_1',\cdots,X_k'\right)$, $1\leq k\leq d-1$ be the canonical filtration genreated by $\{X'_k\}_{k=1}^d$. Since $C(\Omega_1\times\cdots\times\Omega_k)$ is dense in the space of $\calF_k'$-measurable integrable function on  $\Omega_1\times\cdots\times\Omega_k$, by the compactness of $\Omega_1\times\cdots\times\Omega_k$ and Dominance Convergence Theorem, the equation \eqref{mart_alpha} implies
\begin{equation}\label{eq.mart_constraint}
\EE_{\bX'\sim \pi}\left[X'_{k+1}|\calF_k'\right] = X_k' \quad \pi - a.s. \quad\forall 1\leq k\leq d-1
\end{equation}
Hence $\{X_k'\}_{k=1}^d$ is a martingale under the probability measure $\pi$, which implies $\pi_1\preceq_{c}\cdots\preceq_{c}\pi_d$, where $\pi_k$ is the $k$-th marginal measure of $\pi$ ($1\leq k\leq d$).

Now we turn to the equation \eqref{margin_beta}. For any $1\leq k\leq d$, note that any indicator function of Borel measurable set in $\Omega_k$ can be approximated by functions in $C(\Omega_k)$, similar to the previous argument, by the compactness of $\Omega_k$ and Dominance Convergence Theorem, we have $\bpi_k = \nu_k$ ($1\leq k\leq d$), where $\bpi_k$ is the $k$-th martingale measure of $\bpi$ (note that $\bpi$ is a $2d$-dimensional measure).

For each $1\leq k\leq d$, let $\tilde\bpi_k$ be the restriction of $\bpi$ on its $k$-th martingale and $(d+k)$-th marginal. From the above discussion we know that $\tilde\bpi_k$ is a coupling of $\nu_k$ and $\pi_k$. By equation \eqref{robust_gamma} and the definition of Wasserstein distance, we obtain
\begin{align*}
\sum_{k=1}^d \calW(\nu_k,\pi_k) &\leq \sum_{k=1}^d\int_{\Omega_k\times\Omega_k}|x_k -x_k'|\tilde{\bpi}_k(dx_k, dx_k')\\
&= \int_{\Omega\times\Omega} \sum_{k=1}^d|x_k-x_k'| \bpi(d\bX, d\bX')\leq \varepsilon
\end{align*}
To sum up, given $\bpi\in\bPi$, the inner infimum of the LHS in \eqref{eq.sion-minimax} $\neq -\infty$ if and only if $\pi\in \calP_{(\nu_1,\cdots,\nu_d)}(\varepsilon)$  (note that $\pi$ is the projection of $\bpi$ on $\bX'$). Furthermore, by \eqref{mart_alpha}, \eqref{margin_beta} and \eqref{robust_gamma}, for any $\bpi\in\bPi$ satisfying $\pi\in \calP_{(\nu_1,\cdots,\nu_d)}(\varepsilon)$, we have
\begin{align*}
&\quad \inf_{\mbox{$\begin{subarray}{c}\{\alpha_k\in C(\Omega_1\times\cdots\times\Omega_k)\}_{k=1}^{d-1}\\
\{\beta_k\in C(\Omega_k)\}_{k=1}^{d}\\		
\gamma\ge 0\end{subarray}$}} \calL\left(\bpi,\gamma,\left\lbrace\alpha_k\right\rbrace_{k=1}^{d-1}, \left\lbrace\beta_k\right\rbrace_{k=1}^{d}\right) \\
& = \inf_{\mbox{$\begin{subarray}{c}\{\alpha_k\in C(\Omega_1\times\cdots\times\Omega_k)\}_{k=1}^{d-1}\\
\{\beta_k\in C(\Omega_k)\}_{k=1}^{d}\\		
\gamma\ge 0\end{subarray}$}} \EE_{\bX'\sim\pi}f(\bX') +  \gamma\left(\varepsilon - \int_{\Omega\times\Omega} \sum_{k=1}^d|x_k-x_k'| \bpi(d\bX, d\bX')\right)\\
& = \EE_{\bX'\sim\pi}f(\bX')
\end{align*}
Hence 
\begin{equation}\label{proof.RHS}
\sup_{\bpi \in \bPi} \inf_{\mbox{$\begin{subarray}{c}\{\alpha_k\in C(\Omega_1\times\cdots\times\Omega_k)\}_{k=1}^{d-1}\\
\{\beta_k\in C(\Omega_k)\}_{k=1}^{d}\\		
\gamma\ge 0\end{subarray}$}} \calL\left(\bpi,\gamma,\left\lbrace\alpha_k\right\rbrace_{k=1}^{d-1}, \left\lbrace\beta_k\right\rbrace_{k=1}^{d}\right) =  I_{(\nu_1,\cdots,\nu_d)}(f;\varepsilon)
\end{equation}

On the other hand, an alternative expression of $\calL$ is
\begin{equation}\label{eq.RHS_Sion}
\begin{aligned}
\calL\left(\bpi,\gamma,\left\lbrace\alpha_k\right\rbrace_{k=1}^{d-1}, \left\lbrace\beta_k\right\rbrace_{k=1}^{d} \right) &= \gamma\varepsilon + \sum_{k=1}^d\int_{\Omega_k}\beta_k(x_k)\nu_k(dx_k) 
+ \int_{\Omega\times\Omega} \left[f\left(\bX'\right)- \sum_{k=1}^{d}\beta_k(x_k)\right.\\
&\left. -\gamma\sum_{k=1}^d|x_k-x_k'| + \sum_{k=1}^{d-1}\alpha_k(x_1',\cdots,x_k')(x_{k+1}'-x_k')\right]\bpi(d\bX, d\bX') 
\end{aligned}
\end{equation}
Therefore, when taking the supremum of $\calL$ over $\bpi\in\bPi$, the probability measure $\bpi$ will pick the supremum of the inner integral in RHS of \eqref{eq.RHS_Sion} over all the $\bX, \bX'\in\Omega$, which implies the following 
\begin{equation*}
\begin{aligned}
&\sup_{\bpi\in\bPi}\calL \left(\bpi,\gamma,\left\lbrace\alpha_k\right\rbrace_{k=1}^{d-1}, \left\lbrace\beta_k\right\rbrace_{k=1}^{d} \right) \\
&= \gamma\varepsilon + \sum_{k=1}^d\int_{\Omega_k}\beta_k(x_k)\nu_k(dx_k) 
+ \sup_{\bX, \bX'\in\Omega}\left\lbrace f\left(\bX'\right)- \sum_{k=1}^{d}\beta_k(x_k)-\gamma\sum_{k=1}^d|x_k-x_k'| + \sum_{k=1}^{d-1}\alpha_k(\bX_k')(x_{k+1}'-x_k')\right\rbrace\\
&= \gamma\varepsilon +  \sum_{k=1}^{d-1}\int_{\Omega_k}\beta_k(x_k)\nu_k(dx_k) 
+ \int_{\Omega_d}\beta_d(x_d)\nu_d(dx_d) + \sup_{x_d\in\Omega_{d}}\left\lbrace F\left(x_d; \gamma, \left\lbrace\alpha_k\right\rbrace_{k=1}^{d-1}, \left\lbrace\beta_k\right\rbrace_{k=1}^{d-1}\right) - \beta_d(x_d)\right\rbrace\\
&=  \gamma\varepsilon +  \sum_{k=1}^{d-1}\int_{\Omega_k}\beta_k(x_k)\nu_k(dx_k) 
+ \int_{\Omega_d}\left[\beta_d(x_d) + \sup_{x_d\in\Omega_{d}}\left\lbrace F\left(x_d; \gamma, \left\lbrace\alpha_k\right\rbrace_{k=1}^{d-1}, \left\lbrace\beta_k\right\rbrace_{k=1}^{d-1}\right) - \beta_d(x_d)\right\rbrace \right]\nu_d(dx_d)\\
&\geq \gamma\varepsilon +  \sum_{k=1}^{d-1}\int_{\Omega_k}\beta_k(x_k)\nu_k(dx_k) 
+ \int_{\Omega_d} F\left(x_d; \gamma, \left\lbrace\alpha_k\right\rbrace_{k=1}^{d-1}, \left\lbrace\beta_k\right\rbrace_{k=1}^{d-1}\right)\nu_d(dx_d)
\end{aligned}
\end{equation*}
where 
\begin{equation}
\begin{aligned}
F\left(x_d; \gamma, \left\lbrace\alpha_k\right\rbrace_{k=1}^{d-1}, \left\lbrace\beta_k\right\rbrace_{k=1}^{d-1}\right) : = \sup_{\mbox{$\begin{subarray}{c} x_k\in\Omega_k, 1\leq k\leq d-1\\
\bX'\in\Omega\end{subarray}$}}\left\lbrace f\left(\bX'\right)- \sum_{k=1}^{d-1}\beta_k(x_k)-\gamma\sum_{k=1}^{d}|x_k-x_k'| + \right. \\ 
\left.  \sum_{k=1}^{d-1}\alpha_k(\bX_k')(x_{k+1}'-x_k')\right\rbrace
\end{aligned}
\end{equation}
To simplify the notation, we abbreviate the above function by $F(x_d)$ in the rest of the proof. Now, let $\calS$ denotes the feasible set of $J_{(\nu_1,\cdots,\nu_d)}(\varepsilon)$ which consist of $(\gamma,\left\lbrace\alpha_k\right\rbrace_{k=1}^{d-1}, \left\lbrace\beta_k\right\rbrace_{k=1}^{d})$ that satisfying the constraints stated in Theorem \ref{thm.strongdual}. 
Now  RHS of \eqref{eq.sion-minimax} is lower bounded by
\begin{equation}\label{strongdual_I>=J}
\begin{aligned}
&\inf_{\mbox{$\begin{subarray}{c}\{\alpha_k\in C(\Omega_1\times\cdots\times\Omega_k)\}_{k=1}^{d-1}\\
\{\beta_k\in C(\Omega_k)\}_{k=1}^{d}\\		
\gamma\ge 0\end{subarray}$}}\sup_{\bpi \in \bPi} \calL\left(\bpi,\gamma,\left\lbrace\alpha_k\right\rbrace_{k=1}^{d-1}, \left\lbrace\beta_k\right\rbrace_{k=1}^{d}\right) \\
%&\geq \inf_{\mbox{$\begin{subarray}{c}\{\alpha_k\in C(\Omega_1\times\cdots\times\Omega_k)\}_{k=1}^{d-1}\\
%\{\beta_k\in C(\Omega_k)\}_{k=1}^{d}\\		
%\gamma\ge 0\end{subarray}$}} \gamma\varepsilon +  \sum_{k=1}^{d-1}\int_{\Omega_k}\beta_k(x_k)\nu_k(dx_k) 
%+ \int_{\Omega_d} G(x_d)\nu_d(dx_d)\\
&= \inf_{(\gamma,\left\lbrace\alpha_k\right\rbrace_{k=1}^{d-1}, \left\lbrace\beta_k\right\rbrace_{k=1}^{d-1},F(x_d))\in\calS} \gamma\varepsilon +  \sum_{k=1}^{d-1}\int_{\Omega_k}\beta_k(x_k)\nu_k(dx_k) 
+ \int_{\Omega_d} F(x_d)\nu_d(dx_d)\\
&\geq J_{(\nu_1,\cdots,\nu_d)}(\varepsilon)
\end{aligned}
\end{equation}

Combining the above equation \eqref{strongdual_I>=J} with equation \eqref{proof.RHS}, we have $I_{(\nu_1,\cdots,\nu_d)}(\varepsilon)\geq J_{(\nu_1,\cdots,\nu_d)}(\varepsilon)$, which yield the strong duality. Finally, it is not hard to see that $\calP_{(\nu_1,\cdots,\nu_d)}(\varepsilon)$ is compact in $\bPi$ with respect to weak topology, thus there exist a primal optimizer $\pi^*\in\calP_{(\nu_1,\nu_2,\cdots,\nu_d)}(\varepsilon)$ for $I_{(\nu_1,\cdots,\nu_d)}(f;\varepsilon)$.
\end{proof}
\begin{corollary}\label{cor.dual_reformulation}
Suppose $\Omega_k$ are compact subsets of $\RR$, let $\nu_k\in\calP(\Omega_k)$, $k=1,2,\cdots, d$. Given $\varepsilon>0$ such that $\calP_{(\nu_1,\nu_2,\cdots,\nu_d)}(\varepsilon)\ne\varnothing$, we have 
\begin{equation}\label{eq.dual_reformulation}
I_{(\nu_1,\cdots,\nu_d)}(f;\varepsilon) = 
\inf_{\left(\gamma, \left\lbrace\alpha_k\right\rbrace_{k=1}^{d-1}, \left\lbrace\beta_k\right\rbrace_{k=1}^{d-1}\right)\in\calS_{(\nu_1,\cdots,\nu_{d-1})}(\varepsilon)}\gamma\varepsilon + \int_{\Omega_d}
F\left(x_d; \gamma, \left\lbrace\alpha_k\right\rbrace_{k=1}^{d-1}, \left\lbrace\beta_k\right\rbrace_{k=1}^{d-1}\right)\nu_d(dx_d)
\end{equation}	
where  
\begin{equation}\label{keyFunction}
\begin{aligned}
F\left(x_d; \gamma, \left\lbrace\alpha_k\right\rbrace_{k=1}^{d-1}, \left\lbrace\beta_k\right\rbrace_{k=1}^{d-1}\right) : = \sup_{\mbox{$\begin{subarray}{c} x_k\in\Omega_k, 1\leq k\leq d-1\\
\bX'\in\Omega\end{subarray}$}}\left\lbrace f\left(\bX'\right)- \sum_{k=1}^{d-1}\beta_k(x_k)-\gamma\sum_{k=1}^{d}|x_k-x_k'| + \right. \\ 
\left.  \sum_{k=1}^{d-1}\alpha_k(\bX_k')(x_{k+1}'-x_k')\right\rbrace
\end{aligned}
\end{equation}
and 
\begin{align*}
\calS_{(\nu_1,\cdots,\nu_{d-1})}(\varepsilon) := \left\lbrace \left(\gamma, \left\lbrace\alpha_k\right\rbrace_{k=1}^{d-1}, \left\lbrace\beta_k\right\rbrace_{k=1}^{d-1}\right) : \gamma\geq 0, \alpha_k\in C(\Omega_1\times\cdots\times\Omega_k), \beta_k\in C(\Omega_k), \right.\\
\left. \int_{\Omega_k}\beta_k(x)\nu_k(dx) = 0, \emph{ for all }1\leq k\leq d-1 \right\rbrace
\end{align*} 
\end{corollary}
\begin{proof}
To simply the notation, we use $F(x_d)$ as an abbreviation of $F\left(x_d; \left\lbrace\alpha_k\right\rbrace_{k=1}^{d-1}, \left\lbrace\beta_k\right\rbrace_{k=1}^{d-1}\right)$. In the proof of Theorem \ref{thm.strongdual}, we've actually obtained the following result (see \eqref{strongdual_I>=J})
\begin{equation}\label{cor1.keyexpression}
I_{(\nu_1,\cdots,\nu_d)}(f;\varepsilon) = \inf_{\mbox{$\begin{subarray}{c}\gamma \geq 0, \alpha_k\in C(\Omega_1\times\cdots\times\Omega_k), \\
\beta_k\in C(\Omega_k), 1\leq k\leq d-1\end{subarray}$}} \gamma\varepsilon + \sum_{k=1}^{d-1}\int_{\Omega_k}\beta_{k}(x)\nu_k(dx) + \int_{\Omega_d}
F\left(x_d\right)\nu_d(dx_d)
\end{equation}
By the definition of $F$, we oberve that the obejecive value $I_{(\nu_1,\cdots,\nu_d)}(f;\varepsilon)$ won't changed when shifting any $\beta_k(\cdot)$ to $\beta_k(\cdot) + \lambda_k$ by an arbitrary constant $\lambda_k$. Hence we can properly select constants $\lambda_k$ $(1\leq k\leq d-1)$ to enforce the constraints
\begin{equation*}
\int_{\Omega_k}\beta_k(x)\nu_k(dx) = 0, \textrm{ for all }1\leq k\leq d-1
\end{equation*}
Plugging the above constraints into \eqref{cor1.keyexpression}, we conclude the desired result.
\end{proof}
\begin{remark}
By symmetry, we can replace $\nu_d$ in \eqref{eq.dual_reformulation} by any other $\nu_k$ $(1\leq k\leq d-1)$, and the Corollary \ref{cor.dual_reformulation} still holds after we adjust the definition of $F$ and $\calS$ accordingly.
\end{remark}

==> formulation.tex <==
We first introduces some notations and definitions that will be frequently used in this paper.  Let $\Omega$ be a subset of $\RR^d$, and $\calP(\Omega)$ denotes 
the set of all probability measures supported on $\Omega$.  
%Let$c(\cdot,\cdot):\RR^d\times\RR^d\rightarrow\RR_{\geq0}$ be a distance function, 
For any probability distributions $\mu$ and $\nu$ supported on $\RR^d$, we can define the Wasserstein distance between $\mu$ and $\nu$ as
\begin{equation}
\begin{aligned}
\calW(\mu,\nu) :&=\inf_{\pi\in\Pi(\mu,\nu)}\iint_{\RR^d\times\RR^d}|x-y|d\pi(x,y)\\
&= \sup_{f\in\textrm{Lip}_1(\RR^d)} \left\lbrace \int_{\RR^d} f(x)d\mu(x) - \int_{\RR^d} f(x)d\nu(x)\right\rbrace 
\end{aligned}
\end{equation}


In our paper, we focus on the distributional uncertainty set that induced by Wasserstein distance $\calW(\cdot,\cdot)$. Let $\mathbf{X}:=(X_1, X_2,\cdots,X_d)\in\RR^d$ be a $d$ dimensional random vector represents a $d$-period price process with support begin $\Omega = \prod_{i=1}^d\Omega_i$ ($\Omega_i\subset\RR$), and it follows a probability law $\pi^*\in\Pi(\mu_1,\cdots,\mu_d)$, which is presumably inaccessible while we only made really weak assumptions on it, namely the price process of the underlying is a martingale (to rule out the arbitrage opportunities) and its marginals $\mu_i\in\calP(\Omega_i)$ ($1\leq i\leq d$) are given by the observation of European Call prices (via the so-called Breeden-Litzenberger formula). 

Denoted by $\mu\preceq_c\nu$, we say two probability distribution $\mu$ and $\nu$ are in convex ordering if and only if 
\begin{equation}
\int\phi(x)\mu(dx) \leq \int\phi(x)\nu(dx)
\end{equation}
holds for arbitrary convex function $\phi$. Furthermore, we define the uncertainty set $\calP_{(\mu_1,\mu_2,\cdots,\mu_d)}(\varepsilon)$ as :
\begin{equation}\label{uncertaintyset}
\calP_{(\mu_1,\mu_2,\cdots,\mu_d)}(\varepsilon):= \left\lbrace \pi\in\calP\left(\Pi_{i=1}^d\Omega_i\right):  \pi\textrm{ is a martingale measure},  \sum_{i=1}^d\calW(\mu_i,\pi_i)\leq\varepsilon\right\rbrace
\end{equation}
where $\pi_i$ is the $i$th marginal of $\pi$ (we will keep this notation in the rest of the paper). 

For each $i$, we always assume that we can observe i.i.d samples $X_i^{(1)}, X_i^{(2)}, \cdots$ from $\mu_i$, and $\widehat{\mu}_i^{(n)}$ denotes the empirical distribution function,
\begin{equation}\label{defn.empirical_distribution}
\widehat{\mu}_i^{(n)}(dx):=\frac{1}{n}\sum_{j=1}^n\mathbbm{1}(X_i^{(j)}\in dx)
\end{equation}
In this paper, we want to solve the following problem:
\\
\\
For a fixed  $\varepsilon>0$, compute (approximately) the following distributionally robust worst-case expectation with martingale constraint:
\begin{equation}\label{eq.worstcase}
I_{(\mu_1,\cdots,\mu_d)}(f;\varepsilon) := 
\sup_{\pi\in\calP_{(\mu_1,\mu_2,\cdots,\mu_d)}(\varepsilon)}\EE_{\pi}\left[f(\bX)\right]
\end{equation}
The worst-case expectation in \eqref{eq.worstcase} is a infinite dimensional LP which can not be solved directly. We proposed a two step ``discretization'' to approximately solve this problem. (\myworries{TODO: Discuss the connection with classical martingale transport})

First of all we introduce the worst-case expectation problem in below, in which we replace the $\mu_i$'s in \eqref{eq.worstcase} by  $\widehat{\mu}_i^{(n)}$'s,
\begin{equation}\label{eq.empiricalworstcase}
I_{\left(\widehat{\mu}_1^{(n)},\widehat{\mu}_2^{(n)},\cdots,\widehat{\mu}_d^{(n)}\right)}(f;\varepsilon) := 
\sup_{\pi\in\calP_{\left(\widehat{\mu}_1^{(n)},\widehat{\mu}_2^{(n)},\cdots,\widehat{\mu}_d^{(n)}\right)}(\varepsilon)}\EE_{\pi}\left[f(\bX)\right]
\end{equation}
we will show that $I_{\left(\widehat{\mu}_1^{(n)},\widehat{\mu}_2^{(n)},\cdots,\widehat{\mu}_d^{(n)}\right)}(\varepsilon)$ is a good approximation of $I_{(\mu_1,\cdots,\mu_d)}(\varepsilon)$  and then try to approximately solve \eqref{eq.empiricalworstcase} (note that the worst-case expectation \eqref{eq.empiricalworstcase} still can't be solved directly (say, by a LP solver) in our setting).

Throughout the paper, we assume that
\begin{assumption}\label{aspn.convexorder}
	The undering probability measure $\pi^*\in\Pi(\mu_1,\cdots,\mu_d)$ is a martingale measure in $\RR^d$. Consequently, $\left\lbrace \mu_i\right\rbrace_{i=1}^d$ follow the convex ordering, i.e., $\mu_1\preceq_{c}\cdots\preceq_{c}\mu_d$.
\end{assumption}

\begin{assumption}\label{aspn.cost_function} The  cost function $f(\bX)$ is a $L-$Lipschitz function in $\RR^d$.
\end{assumption}

==> stability_compact.tex <==
In this subsection we study the stability of the robust worse case problem 
\begin{equation*}
I_{(\nu_1,\cdots,\nu_d)}(f;\varepsilon) = 
\sup_{\pi\in\calP_{(\nu_1,\nu_2,\cdots,\nu_d)}(\varepsilon)}\EE_{\bX\sim \pi}\left[f(\mathbf{X})\right]
\end{equation*}	
with respect to its marginals as well as the uncertainty radius $\varepsilon$.

\begin{prop}
Given $\nu_i\in\calP(\Omega_i)$, 
\leavevmode
\begin{enumerate}	
\item [\emph{(1)}]  Let $\calR_{(\nu_1,\cdots,\nu_d)} := \inf\{\varepsilon \geq 0 : \calP_{(\nu_1,\nu_2,\cdots,\nu_d)}(\varepsilon)\neq\varnothing\}$, then $I_{(\nu_1,\cdots,\nu_d)}(f;\varepsilon)$ is both concave and continuous as a function of  $\varepsilon\in (\calR_{(\nu_1,\cdots,\nu_d)}, +\infty)$
\item [\emph{(2)}] In particular, if $\nu_1\leq_c\cdots\leq_c\nu_d$, then $I_{(\nu_1,\cdots,\nu_d)}(f;\varepsilon)$ is a continuous function of $\varepsilon\in [0, +\infty)$
\end{enumerate}
\end{prop}

\begin{proof}
\leavevmode
\begin{enumerate}
\item[(1)] First of all, note that $I_{(\nu_1,\cdots,\nu_d)}(f;\varepsilon) < \infty$ when  $\varepsilon\in (\calR_{(\nu_1,\cdots,\nu_d)}, +\infty)$. For any $\varepsilon_1,\varepsilon_2\in (\calR_{(\nu_1,\cdots,\nu_d)}, +\infty)$ and $t\in[0,1]$, we claim the following inequality holds
\begin{equation}\label{eq.prop.stability_varepsilon_final}
I_{(\nu_1,\cdots,\nu_d)}(f; t\varepsilon_1 + (1-t)\varepsilon_2) \geq tI_{(\nu_1,\cdots,\nu_d)}(f;\varepsilon_1) + (1-t)I_{(\nu_1,\cdots,\nu_d)}(f;\varepsilon_2)
\end{equation}
Pick any $\pi^{(1)}\in \calP_{(\nu_1,\nu_2,\cdots,\nu_d)}(\varepsilon_1)$ and  $\pi^{(2)}\in \calP_{(\nu_1,\nu_2,\cdots,\nu_d)}(\varepsilon_2)$, we define a new probability measure $\widetilde{\pi} := t\pi_1 + (1-t)\pi_2$.  Let $\widetilde{\pi}_i$ denotes the $i$th marginal of $\widetilde{\pi}$ ($1\leq i\leq d$), note that
\begin{align*}
\sum_{i=1}^d \calW\left(\tilde{\pi}_i, \nu_i\right) &=  \sum_{i=1}^d \sup_{f\in\textrm{Lip}_1} \left\lbrace \int fd\widetilde{\pi}_i - \int fd\nu_i\right\rbrace \\
&\leq \sum_{i=1}^d t\sup_{f\in\textrm{Lip}_1} \left\lbrace \int fd\widetilde{\pi}^{(1)}_i - \int fd\nu_i\right\rbrace + (1-t)\sum_{i=1}^d \sup_{f\in\textrm{Lip}_1} \left\lbrace \int fd\widetilde{\pi}^{(2)}_i - \int fd\nu_i\right\rbrace\\
&= t\sum_{i=1}^d\calW\left(\widetilde{\pi}^{(1)}_i, \nu_i\right) + (1-t) \sum_{i=1}^d\calW\left(\widetilde{\pi}^{(2)}_i, \nu_i\right)\\
&\leq t\varepsilon_1 + (1-t)\varepsilon_2
\end{align*}
It remains to check $\widetilde{\pi}_i$'s are in convex ordering. This follows from the fact that, for any $1\leq i\leq d-1$, we have 
\begin{align*}
\int \phi d\widetilde{\pi}_i &= t\int \phi d\pi^{(1)}_i + (1-t)\int \phi d\pi^{(2)}_i\leq t\int \phi d\pi^{(1)}_{i+1} + (1-t)\int \phi d\pi^{(2)}_{i+1} = \int \phi d\widetilde{\pi}_{i+1}
\end{align*}
holds for abitrary convex function $\phi$. Thus we just showed that  $\widetilde{\pi}\in  \calP_{(\nu_1,\nu_2,\cdots,\nu_d)}(t\varepsilon_1 + (1-t)\varepsilon_2)$, and as a result we have
\begin{equation}\label{eq.prop.stability_varepsilon}
I_{(\nu_1,\cdots,\nu_d)}(f; t\varepsilon_1 + (1-t)\varepsilon_2) \geq \EE_{\bX\sim\widetilde{\pi}}f(\bX) = t\EE_{\bX\sim\pi_1}f(\bX) + (1-t) \EE_{\bX\sim\pi_2}f(\bX)
\end{equation}
Take the supremum of RHS of \eqref{eq.prop.stability_varepsilon} over $\pi^{(1)}\in \calP_{(\nu_1,\nu_2,\cdots,\nu_d)}(\varepsilon_1)$ and  $\pi^{(2)}\in \calP_{(\nu_1,\nu_2,\cdots,\nu_d)}(\varepsilon_2)$, we prove the desired inequality in \eqref{eq.prop.stability_varepsilon_final}, and thus $I_{(\nu_1,\cdots,\nu_d)}(f; \varepsilon)$ is concave and continuous.
\item [(2)] It suffices to show that $I_{(\nu_1,\cdots,\nu_d)}(f;\varepsilon)$ is right continuous at 0. Take any sequence $\varepsilon_n\rightarrow0$, and $\pi^{(n)}\in\calP_{(\nu_1,\cdots,\nu_d)}(\varepsilon_n)$ that optimize $I_{(\nu_1,\cdot,\nu_d)}(f;\varepsilon_n)$. Observe that 
\begin{align*}
\sup_{n\geq 1}\EE_{\bX\sim\pi^{(n)}}|\bX|&\leq \sup_{n\geq1}\left\lbrace \sum_{i=1}^d \int|x|\pi_i^{(n)}(dx)\right\rbrace \\
&\leq \sup_{n\geq1}\left\lbrace \sum_{i=1}^d \int|x|\nu_i(dx) + \sum_{i=1}^d\calW\left(\pi_i^{(n)},\nu_i\right)\right\rbrace\\
&\leq \sum_{i=1}^dm_1(\nu_i) + \sup_{n\geq 1}\varepsilon_n <\infty.
\end{align*}
\end{enumerate}
Hence $\left\lbrace\pi^{(n)}\right\rbrace_{n\geq 1}$ is uniformly tight, we may assume they converge weakly to a probability measure $\pi\in\Pi(\nu_1,\cdots,\nu_d)$ without loss of generality. Moreover, for every $k=1,2,\cdots,d-1$, we have 
\begin{equation*}
\EE_{\bX\sim\pi^{(n)}}\left[\alpha_k(X_1,\cdots,X_k)(X_{k+1}-X_k)\right] = 0, \quad n\geq1.
\end{equation*}
holds for every continuous function $\alpha_k(\cdot)$ on $\Omega_1\cdots\Omega_k$. Follows from the Dominated Convergence Theorem we have the above equalities also holds for $\pi$, which implies $\pi\in\calP_{\nu_1,\cdots,\nu_d}(0)$. As a result,
\begin{equation*}
\limsup_{n\rightarrow\infty}I_{(\nu_1,\cdots,\nu_d)}(f;\varepsilon_n) = \limsup_{n\rightarrow} \EE_{\bX\sim\pi^{(n)}}f(\bX) = \EE_{\bX\sim\pi}f(\bX)\leq I_{(\nu_1,\cdots,\nu_d)}(f;0)
\end{equation*}
The reverse inequality holds trivially from the definition.
\end{proof}

Next we discuss the stability of $I_{(\nu_1,\cdots,\nu_d)}(f; \varepsilon)$ with respect to the marginals. In particular, we study the convergence of 
$I_{\left(\widehat{\mu}_1^{(n)},\widehat{\mu}_2^{(n)},\cdots,\widehat{\mu}_d^{(n)}\right)}(f;\varepsilon) $ to $I_{(\mu_1,\cdots,\mu_d)}(f;\varepsilon)$, where $\widehat{\mu}_i^{(n)}$ are empirical distributions defined in \eqref{defn.empirical_distribution}. Since $\widehat{\mu}_i^{(n)}$ $(1\leq i\leq d)$ are not necessarily follows the convex ordering.  We first show that the Robust Martingale DRO problem \eqref{eq.empiricalworstcase} is feasible with high probability as long as $n \gtrsim \varepsilon^{-2}$: 
 
 \begin{lemma}\label{lemma.feasibility}
 Under Assumption \ref{aspn.convexorder} and \ref{aspn.compact_support}, for any  $\varepsilon>0$ and $\delta\in(0,1)$, there exist universal constants $C_1,  C_2>0$ such that the Robust Martingale DRO problem \eqref{eq.empiricalworstcase} is feasible with probability $1-\delta$ when $n\geq N(\varepsilon,\delta):= \frac{d^2}{C_2}\log\left(\frac{dC_1}{\delta}\right)\varepsilon^{-2}$.
 	
 \begin{proof}
 The optimization problem \eqref{eq.empiricalworstcase} is feasible if and only if $\calP_{\left(\widehat{\mu}_1^{(n)},\widehat{\mu}_2^{(n)},\cdots,\widehat{\mu}_d^{(n)}\right)}(\varepsilon)\neq \varnothing$. By Assumption \ref{aspn.compact_support}, each marginal probability $\mu_i$ of true underlying martingale measure $\pi^*$ has a finite square-exponential moment, thus we can apply the Theorem 2 in \cite{fournier2015rate} to conclude:
 \begin{equation}\label{eq.concentrateEm}
 \PP\left(\sum_{i=1}^d\calW(\widehat{\mu}_i^{(n)},\mu_i)>\varepsilon\right)\leq\sum_{i=1}^d\PP\left(\calW(\widehat{\mu}_i^{(n)},\mu_i)>\frac{\varepsilon}{d}\right)\leq dC_1e^{-C_2n\varepsilon^2/d^2}<\delta
 \end{equation}
holds when $n\geq N(\varepsilon,\delta)$, thus $\pi^*\in\calP_{\left(\widehat{\mu}_1^{(n)},\widehat{\mu}_2^{(n)},\cdots,\widehat{\mu}_d^{(n)}\right)}(\varepsilon)$ with probability at least $1-\delta$, which yields the desired result.
 \end{proof}
 \end{lemma}

Next we show the consistency of  $I_{\left(\widehat{\mu}_1^{(n)},\widehat{\mu}_2^{(n)},\cdots,\widehat{\mu}_d^{(n)}\right)}(f;\varepsilon)$, with convergence rate is at most  $\calO(1/n^{1/2})$.

\begin{theorem}\label{thm.distance_n}
Under Assumptions \ref{aspn.convexorder} and \ref{aspn.compact_support}, for any $\varepsilon>0$, $\delta\in(0,1)$ and $n\geq N\left(\frac{\varepsilon}{2},\frac{\delta}{2d}\right)$ (defined in Lemma \ref{lemma.feasibility}) , with probability at least $1-\delta$ we have
\begin{equation}
\left|I_{\left(\widehat{\mu}_1^{(n)},\widehat{\mu}_2^{(n)},\cdots,\widehat{\mu}_d^{(n)}\right)}(f;\varepsilon) - I_{(\mu_1,\cdots,\mu_d)}(f;\varepsilon)\right|\le \frac{4d}{\varepsilon}\sqrt{\frac{\log\left(2C_1d/\delta\right)}{C_2n}}\sup_{\bX\in\Omega}\left|f(\bX)\right|
\end{equation}
where the universal constants $C_1, C_2>0$ are defined in Lemma \ref{lemma.feasibility}.
\end{theorem}

\begin{proof}
Let $\boldsymbol{\mu}_0$, $\boldsymbol{\mu}_d$ denotes  $\left(\widehat{\mu}_1^{(n)},\widehat{\mu}_2^{(n)},\cdots,\widehat{\mu}_d^{(n)}\right)$, $(\mu_1,\cdots,\mu_d)$  correspondingly, and $\boldsymbol{\mu}_k$ denotes $(\widehat{\mu}_{1},\cdots, \widehat{\mu}_{d-k}, \mu_{d-k+1},\cdots,\mu_d)$ for $1\leq k\leq d-1$, . By triangular inequality we have 
\begin{equation}\label{thm2.triangular}
\left|I_{\left(\widehat{\mu}_1^{(n)},\widehat{\mu}_2^{(n)},\cdots,\widehat{\mu}_d^{(n)}\right)}(f;\varepsilon) - I_{(\mu_1,\cdots,\mu_d)}(f;\varepsilon)\right| = \left|I_{\boldsymbol{\mu}_0}(f;\varepsilon) - I_{\boldsymbol{\mu}_d}(f;\varepsilon)\right| \leq \sum_{k=0}^{d-1} \left|I_{\boldsymbol{\mu}_k}(f;\varepsilon) - I_{\boldsymbol{\mu}_{k+1}}(f;\varepsilon)\right|
\end{equation}
Since for each $k$, $\boldsymbol{\mu}_k$ and $\boldsymbol{\mu}_{k+1}$ are only different from  one marginal, by symmetry we just need to bound one of the $d$ terms in \eqref{thm2.triangular}, say $\left| I_{\boldsymbol{\mu}_0}(f;\varepsilon) - I_{\boldsymbol{\mu}_1}(f;\varepsilon)\right|$.

%Note that $\boldsymbol{\mu}_0 = \left(\widehat{\mu}_1^{(n)},\widehat{\mu}_2^{(n)},\cdots,\widehat{\mu}_d^{(n)}\right)$ and $\boldsymbol{\mu}_1 = \left(\widehat{\mu}_1^{(n)},\widehat{\mu}_2^{(n)},\cdots,\widehat{\mu}_{d-1}^{(n)},\mu_d\right)$. 
\noindent Applying Corollary \ref{cor.dual_reformulation} and Lemma  \ref{lemma.feasibility}, for all $n\geq N(\varepsilon,\delta)$, with probability at least $1-\delta$ we have 
\begin{equation}\label{eq.I_mu0}
I_{\boldsymbol{\mu}_0}(f;\varepsilon) =  \inf_{\left(\gamma, \left\lbrace\alpha_k\right\rbrace_{k=1}^{d-1}, \left\lbrace\beta_k\right\rbrace_{k=1}^{d-1}\right)\in\calS_{\left(\widehat{\mu}_1^{(n)},\widehat{\mu}_2^{(n)},\cdots,\widehat{\mu}_{d-1}^{(n)}\right)}(\varepsilon)}\gamma\varepsilon + \int_{\Omega_d}
F\left(x_d; \gamma, \left\lbrace\alpha_k\right\rbrace_{k=1}^{d-1}, \left\lbrace\beta_k\right\rbrace_{k=1}^{d-1}\right)\widehat{\mu}_d^{(n)}(dx_d)
\end{equation}
To simplify the notation, let  $\calS(\varepsilon)$ denotes $\calS_{\left(\widehat{\mu}_1^{(n)},\widehat{\mu}_2^{(n)},\cdots,\widehat{\mu}_{d-1}^{(n)}\right)}(\varepsilon)$. The next step is to show that $F$ is Lipschitz $x_d$. Given $B>0$, we define
\begin{equation}\label{eq.dual_of_I_leq_B}
I_{\boldsymbol{\mu}_0}^{\leq B}(f;\varepsilon) := \inf_{\mbox{$\begin{subarray}{c}\left(\gamma, \left\lbrace\alpha_k\right\rbrace_{k=1}^{d-1}, \left\lbrace\beta_k\right\rbrace_{k=1}^{d-1}\right)\in\calS(\varepsilon),\\
0\leq\gamma\leq B \end{subarray}$}}\gamma\varepsilon + \int_{\Omega_d}
F\left(x_d; \gamma, \left\lbrace\alpha_k\right\rbrace_{k=1}^{d-1}, \left\lbrace\beta_k\right\rbrace_{k=1}^{d-1}\right)\widehat\mu_d^{(n)}(dx_d)
\end{equation}
and 
\begin{equation}
I_{\boldsymbol{\mu}_0}^{> B}(f;\varepsilon) := \inf_{\mbox{$\begin{subarray}{c}\left(\gamma, \left\lbrace\alpha_k\right\rbrace_{k=1}^{d-1}, \left\lbrace\beta_k\right\rbrace_{k=1}^{d-1}\right)\in\calS(\varepsilon),\\
\gamma> B \end{subarray}$}}\gamma\varepsilon + \int_{\Omega_d}
F\left(x_d; \gamma, \left\lbrace\alpha_k\right\rbrace_{k=1}^{d-1}, \left\lbrace\beta_k\right\rbrace_{k=1}^{d-1}\right)\widehat{\mu}_d^{(n)}(dx_d)
\end{equation}
It is easy to see that $I_{\boldsymbol{\mu}_0}^{\leq B}(f;\varepsilon)$ is upper bounded by $\sup_{\bX\in\Omega}f(\bX)$ (simply set all the parameters equals zero).
Besides, by the definition of $F$ we see that
\begin{equation}
\begin{aligned}
I_{\boldsymbol{\mu}_0}^{> B}(f;\varepsilon) \geq \inf_{\mbox{$\begin{subarray}{c}\left(\gamma, \left\lbrace\alpha_k\right\rbrace_{k=1}^{d-1}, \left\lbrace\beta_k\right\rbrace_{k=1}^{d-1}\right)\in\calS(\varepsilon),\\
\gamma> B \end{subarray}$}}\gamma\varepsilon + \int\left(\int\left( f\left(\bX'\right)- \sum_{k=1}^{d-1}\beta_k(x_k)-\gamma\sum_{k=1}^{d}|x_k-x_k'| + \right.\right. \\ 
\left.\left. \sum_{k=1}^{d-1}\alpha_k(\bX_k')(x_{k+1}'-x_k')\right)\bpi\left(d\bX_{-d}, d\bX' \mid x_d\right)\right)\widehat{\mu}_d^{(n)}(dx_d)
\end{aligned}
\end{equation}
holds for every conditional probability measure $\bpi(d\bX_{-d},d\bX'\mid x_d)$, where $d\bX_{-d}$ stands for $(dx_1,\cdots, dx_{d-1})$. By the theory in the standard Martinagle Optimal Transport, there exists an martingale measure $\pi\in\Pi(\mu_1,\cdots,\mu_d)$ that optimize $I_{(\mu_1,\cdots,\mu_d)}(f;0)$. 
In particular, we can pick the $\bpi(d\bX_{-d}, d\bX‘ \mid x_d)$ such that its projection on $\bX'$ is $\pi$, and its projection on $\bX_{-d}$ is a $(d-1)$- dimensional probability measure with marginals $\widehat{\mu}_1^{(n)},\cdots,\widehat{\mu}_{d-1}^{(n)}$. Taking supremum over these $\bpi$'s, and note that $\pi$ is a martingale measure, we have 
\begin{align*}
I_{\boldsymbol{\mu}_0}^{> B}(f;\varepsilon) &\geq \inf_{\mbox{$\begin{subarray}{c}\left(\gamma, \left\lbrace\alpha_k\right\rbrace_{k=1}^{d-1}, \left\lbrace\beta_k\right\rbrace_{k=1}^{d-1}\right)\in\calS(\varepsilon),\\
\gamma> B \end{subarray}$}}\gamma\varepsilon + \EE_{\bX'\sim\pi}f(\bX') - \sum_{k=1}^{d-1}\int_{\Omega_k}\beta_k(x_k)\widehat{\mu}_k^{(n)}(dx_k) + \\
& \qquad\qquad\qquad\qquad\qquad \sum_{k=1}^{d-1}\EE_{\bX'\sim\pi}\left[\alpha_k(\bX_k')(X_{k+1}'-X_k')\right] -\gamma\sum_{k=1}^d\calW\left(\mu_k,\widehat{\mu}_k^{(n)}\right)\\
&\geq \inf_{\mbox{$\begin{subarray}{c}\left(\gamma, \left\lbrace\alpha_k\right\rbrace_{k=1}^{d-1}, \left\lbrace\beta_k\right\rbrace_{k=1}^{d-1}\right)\in\calS(\varepsilon),\\
\gamma> B \end{subarray}$}}\gamma\varepsilon + \EE_{\bX'\sim\pi}f(\bX') - \gamma\sum_{k=1}^d\calW\left(\mu_k,\widehat{\mu}_k^{(n)}\right)\\
&> \EE_{\bX'\sim\pi}f(\bX') + B\left(\varepsilon - \sum_{k=1}^d\calW\left(\mu_k,\widehat{\mu}_k^{(n)}\right)\right)
\end{align*}
By Lemma \ref{lemma.feasibility}, for $n\geq N(\frac{\varepsilon}{2}, \frac{\delta}{2d})$, we see that with probability $1 - \frac{\delta}{2d}$,  
\begin{equation*}
\sum_{k=1}^d\calW\left(\mu_k,\widehat{\mu}_k^{(n)}\right) \leq \frac{\varepsilon}{2}
\end{equation*}
Taking $B = \frac{4}{\varepsilon}\sup_{\bX\in\Omega}\left|f(\bX)\right|$, we have
\begin{align*}
I_{\boldsymbol{\mu}_0}^{> B}(f;\varepsilon) > \EE_{\bX'\sim\pi}f(\bX') + \frac{4}{\varepsilon}\sup_{\bX\in\Omega}\left|f(\bX)\right|\cdot\frac{\varepsilon}{2}>\sup_{\bX\in\Omega}f(\bX)\geq I_{\boldsymbol{\mu}_0}^{\leq B}(f;\varepsilon)
\end{align*}
Hence we have $\gamma$ is bounded by $B$ with high probability. Precisely, we have 
\begin{equation}
I_{\boldsymbol{\mu}_0}(f;\varepsilon) = I_{\boldsymbol{\mu}_0}^{\leq B}(f;\varepsilon) 
\end{equation}
holds with probability at least $1 - \frac{\delta}{2d}$ for $n\geq N(\frac{\varepsilon}{2}, \frac{\delta}{2d})$. Similar arguments can be applied to $I_{\boldsymbol{\mu}_1}(f;\varepsilon)$ and we get 
\begin{equation}
I_{\boldsymbol{\mu}_1}(f;\varepsilon) =  I_{\boldsymbol{\mu}_1}^{\leq B}(f;\varepsilon) 
\end{equation}

\noindent For any $\Delta >0$, there exists $\left(\gamma_{\Delta}, \left\lbrace\alpha_{k,\Delta}\right\rbrace_{k=1}^{d-1}, \left\lbrace\beta_{k,\Delta}\right\rbrace_{k=1}^{d-1}\right)\in\widetilde\calS(\varepsilon)$ such that 
 \begin{equation*}
 \gamma_{\Delta}\varepsilon + \int_{\Omega_d}
 F\left(x_d; \gamma_{\Delta}, \left\lbrace\alpha_{k,\Delta}\right\rbrace_{k=1}^{d-1}, \left\lbrace\beta_{k,\Delta}\right\rbrace_{k=1}^{d-1}\right)\widehat\mu_d^{(n)}(dx_d)\leq I_{\boldsymbol{\mu}_0}(f;\varepsilon) + \Delta
 \end{equation*}
Note that $F(x_d)$ is a $\gamma-$ Lipschitz function for fixed $\gamma$, we have
\begin{align*}
I_{\boldsymbol{\mu}_1}(f;\varepsilon) - I_{\boldsymbol{\mu}_0}(f;\varepsilon) &\leq \gamma_{\Delta}\varepsilon + \int_{\Omega_d}
F\left(x_d; \gamma_{\Delta}, \left\lbrace\alpha_{k,\Delta}\right\rbrace_{k=1}^{d-1}, \left\lbrace\beta_{k,\Delta}\right\rbrace_{k=1}^{d-1}\right)\mu_d(dx_d)\\
& \qquad -\left(\gamma_{\Delta}\varepsilon + \int_{\Omega_d}
F\left(x_d; \gamma_{\Delta}, \left\lbrace\alpha_{k,\Delta}\right\rbrace_{k=1}^{d-1}, \left\lbrace\beta_{k,\Delta}\right\rbrace_{k=1}^{d-1}\right)\widehat\mu_d^{(n)}(dx_d) - \Delta\right)\\
&\leq B\cdot\calW\left(\mu_d,\widehat{\mu}_d^{(n)}\right) + \Delta
\end{align*}
Similarly we have 
$I_{\boldsymbol{\mu}_0}(f;\varepsilon) - I_{\boldsymbol{\mu}_1}(f;\varepsilon)\leq B\cdot\calW\left(\mu_d,\widehat{\mu}_d^{(n)}\right) + \Delta$. Hence $\Delta \rightarrow 0$ yields
\begin{equation}
\left|I_{\boldsymbol{\mu}_0}(f;\varepsilon) - I_{\boldsymbol{\mu}_1}(f;\varepsilon) \right|\leq B\cdot\calW\left(\mu_d,\widehat{\mu}_d^{(n)}\right)
\end{equation}
Recalled from Lemma \ref{lemma.feasibility} that  $\calW\left(\mu_d,\widehat{\mu}_d^{(n)}\right)\leq\sqrt{\frac{\log(2C_1d/\delta)}{C_2n}}$ with probability at least $1-\frac{\delta}{2d}$. Applying the union bound give us 
\begin{equation}\label{eq.thm.stability_bound}
\left|I_{\boldsymbol{\mu}_0}(f;\varepsilon) - I_{\boldsymbol{\mu}_1}(f;\varepsilon) \right|\leq B\sqrt{\frac{\log(2C_1d/\delta)}{C_2n}}
\end{equation}
holds with probability at least $1-\frac{\delta}{d}$ when $n\geq N(\frac{\varepsilon}{2}, \frac{\delta}{2d})$. Finally, similar arguments works for all $\left|I_{\boldsymbol{\mu}_k}(f;\varepsilon) - I_{\boldsymbol{\mu}_{k+1}}(f;\varepsilon) \right|$ and give the same bound as \eqref{eq.thm.stability_bound}, so by once again the union bound, with probability at least $1-\delta$ we have 
\begin{equation}
\left|I_{\left(\widehat{\mu}_1^{(n)},\widehat{\mu}_2^{(n)},\cdots,\widehat{\mu}_d^{(n)}\right)}(f;\varepsilon) - I_{(\mu_1,\cdots,\mu_d)}(f;\varepsilon)\right|\le Bd\sqrt{\frac{\log\left(2C_1d/\delta\right)}{C_2n}}
\end{equation}
holds for $n\geq N(\frac{\varepsilon}{2}, \frac{\delta}{2d})$, which is the desired result.
\end{proof}

